Fundamental tradeoffs between memorization and robustness in random features and neural tangent regimes

This work studies the (non)robustness of two-layer neural networks in various high-dimensional linearized regimes. We establish fundamental trade-offs between memorization and robustness, as measured by the Sobolev-seminorm of the model w.r.t the data distribution, i.e the square root of the average squared $L_2$-norm of the gradients of the model w.r.t the its input. More precisely, if $n$ is the number of training examples, $d$ is the input dimension, and $k$ is the number of hidden neurons in a two-layer neural network, we prove for a large class of activation functions that, if the model memorizes even a fraction of the training, then its Sobolev-seminorm is lower-bounded by (i) $\sqrt{n}$ in case of infinite-width random features (RF) or neural tangent kernel (NTK) with $d \gtrsim n$; (ii) $\sqrt{n}$ in case of finite-width RF with proportionate scaling of $d$ and $k$; and (iii) $\sqrt{n/k}$ in case of finite-width NTK with proportionate scaling of $d$ and $k$. Moreover, all of these lower-bounds are tight: they are attained by the min-norm / least-squares interpolator (when $n$, $d$, and $k$ are in the appropriate interpolating regime). All our results hold as soon as data is log-concave isotropic, and there is label-noise, i.e the target variable is not a deterministic function of the data / features. We empirically validate our theoretical results with experiments. Accidentally, these experiments also reveal for the first time, (iv) a multiple-descent phenomenon in the robustness of the min-norm interpolator.

==> checklist.tex <==
\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See conclusion section of manuscript.}  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{There are none. This is a theoretical piece of work proving fundamental tradeoffs between memorization and robustness.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{In great detail.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{For example, see the statement of Theorem \ref{thm:finiteRFLaw}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplemental.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See description of experiments in section \ref{subsec:expsetup}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See description of experiments in section \ref{subsec:expsetup}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{All experiments run on a laptop.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}
\clearpage

==> clarification.tex <==
Consider a general feature-based model $f(x) = a^\top \Phi(x)$, where $a \in \mathbb R^m$ are cofficients for linearly combining the (possibly random) features $\Phi(x) \in \mathbb R^m$ of an input $x \in \mathbb R^d$. For example, we have $\Phi(x)=x$ and $a=w \in \mathbb R^d$ for a simple linear model; $\Phi(x)=\psi(Wx) \in \mathbb R^k$ and $a=v$ output weights for a two-layer NN with $k$ neurons; $\Phi(x)=(1/\sqrt{k})\psi'(Wx) \otimes x \in \mathbb R^{kd}$ in the NTK; etc. By the Poincar\'e inequality for uniform distribution $\sigma_{d-1}$ on the unit-sphere $\sphere$,
$$
\|\nabla_\sphere f\|_{L^2(\sigma_{d-1})}^2 \ge d\cdot \var_{x \ \sim \sigma_{d-1}}(f(x)) = \var_{x \sim \sigma_{d-1}}(a^\top \sqrt{d}\Phi(x)) = a^\top C a \ge \lambda_{\min}(C)\|a\|^2,
$$
where $C=C(\Phi) \in \mathbb R^{k \times k}$ is the covariance matrix of $\sqrt{d}\Phi(x)$ for $x \sim \sigma_{d-1}$. Thus, the problem of lower-bounding our (non)robustness measure $\|\nabla_{\sphere} f\|_{L^2(\sigma_{d-1})}$ subject to memorization by $f$, of generic data $\mathcal D_n$, is reduced to \emph{(1)} lower-bound smallest eigenvalue of $C$, and \emph{(2)} lower-bound $\|a\|$.
% This is our main insight.

% \vspace{-.5cm}
\paragraph{\emph{(1)} Lower-bounding $\lambda_{\min}(C)$.} This is doable in a variety of scenarios, including the random features (RF) regime with positive-homogeneous activation functions (e.g ReLU) which we demonstrate in our paper for concreteness. Indeed, in such cases, we have $C_{j,\ell}=\|w_j\|\|w_\ell\|\kappa(\frac{w_j^\top}{\|w_j\|} \frac{w_\ell}{\|w_\ell\|})$, a dot-kernel matrix. In various RF and NTK regimes, one can prove via random matrix theory (RMT) arguments in the spirit of [El Karoui '10] that $\lambda_{\min}(C(W))=\Omega(1)$ w.h.p over the choice of $W$.
% , and for $k \asymp d$, and $W \sim N(0,1/d)^{k \times d}$, standard random matrix theory tells us that $C$ and $C^{\mathrm{lin}}:= \alpha R +  \beta WW^\top + \gamma I_k$, have thesame eigenvalue statistics, where $\alpha,\beta,\gamma>0$ with $\gamma= \Omega(1)$. Thus, $\lambda_{\min}(C) = \Omega(1)$ w.p $1-o(1)$. Similar arguments can be applied to prove that $\lambda_{\min}(C) = \Omega(1)$ in the infinite-width NTK regime, or in the finite-width NTK regime when $kd \ge n(\log d)^c$. Note that NTK is a good proxy for NNs learned via gradient-descent.
In fully general scenario, $\lambda_{\min}(C)$ will depend on both data $\mathcal D_n$ and learned hidden weights matrix $W$. % , as explained in manuscript.

\paragraph{\emph{(2)} Lower-bounding $\|a\|$.}
% This where the generic dataset $\mathcal D_n=\{(x_1,y_1),\ldots,(x_n,y_n)\}$ comes in, and
The (ridged) problem is reduced to lower-bounding the trace of the random matrix $R_\lambda(Z):= Q(Q + \lambda I_n)^{-2}$ for $\lambda > 0$, where $Q:=Z^\top Z/n \in \mathbb R^{m \times m}$ with $Z = (\Phi(x_1),\ldots,\Phi(x_n)) \in \mathbb R^{n \times m}$, % and $y=(y_1,\ldots,y_n)$
for a {\bfseries generic dataset} $\mathcal D_n := \{(x_1,y_1),\ldots,(x_n,y_n)\} \equiv (X,y)$. In the case of RF and NTK, nonlinear RMT can be used to obtain $\|a\| = \Omega_{\mathbb P}(\sqrt{n})$ for infinite-width; for finite width, we have $\|a\|=\Omega_{\mathbb P}(\sqrt{n})$ w.p $1-d^{-\Omega(1)}$ (in case of RF) and $\|a\| = \Omega_{\mathbb P}(\sqrt{n/k})$ (for NTK), by careful application of recent RMT techniques in the analysis of neural networks [Mei \& Montanari '19; Montanari \& Zhong '20; Adlam \& Pennington '20].
% $\lambda_{\min}(Q) \ge \mathrm{var}_{N(0,1)}(\sigma'(z))-o_{\mathbb P}(1)=\Omega_{\mathbb P}(1)$.
% For infinite width, one has $\|a\| = \Omega_{\mathbb P}(\sqrt{n})$ via RMT for dot-product kernels.
We thus obtain lower-bounds for $\|\nabla_{\sphere}f\|_{L^2(\sigma_{d-1})}$.
By similar arguments, one can show that all these models memorize $\mathcal D_n$.
% For finite-width, it is easy to show that the min-norm estimator for $a$ memorizes $\mathcal D_n$ almost surely, as soon as $kd = \widetilde{\Omega}(n)$. In the infinite-width case $k=\infty$, memorization is even easier to show.

==> direct.tex <==
% \input{preliminaries.tex}

\section{Homogeneous neural networks: direct analysis (without RKHS trick, etc.)}
\label{sec:hom}
In this section, suppose the activation function $\sigma:\mathbb R \to \mathbb R$ is positive-homogeneous of order $p \ge 0$, i.e $\sigma(ct) = c^p\sigma(t)$ for all $t \in \mathbb R$ and $c \ge 0$. Examples include the power $t^p$; power absolute-value $|t|^p$; power ReLU activation function $\max(t,0)^p$; sign function $\mbox{sign}(t)=1[t \ge 0]$; etc.. As we shall, see homogeneous activation functions allow us to write $\mathfrak{S}(f_{W,v})^2$ as a quadratic form $v^\top C_\sigma(W) v$, for a psd matrix $C_\sigma(W)$ which only depends on $W$ and $\sigma$. Thus, if we control the extreme eigenvalues of $C_\sigma(W)$, then we can obtain lower- and upper-bounds on $\mathfrak{S}(f_{W,v})^2$ as a scalar multiple of $\|v\|^2$, more precisely
$$
\lambda_{\min}(C_\sigma(W))\|v\|^2 \le\mathfrak{S}(f_{W,v})^2 \le \lambda_{\max}(C_\sigma(W))\|v\|^2.
$$
Finally, for $f_{W,v}$ which memorizes generic data $\mathcal D_n$, we shall obtain lower-bounds on $\|v\|$, thus given lower bounds for $\mathfrak{S}(f_{W,v})$.

% \mytodo{Still not clear what "under(over)determined" means here!}
% \paragraph{Over-determined case: $n > d$ (i.e $\delta > 1$).}
% In this case, the unique solution is $\widehat{w}_{OLS} = (X^\top X)^{-1}X^\top y$, with squared norm $\|\widehat{w}_{OLS}\|^2 = y^\top (X^\top X)^{-1} y \ge \|y\|^2/\lambda_{\max}(X^\top X) \ge \Omega(1)\cdot \|y\|^2$ w.p $1-A'e^{-B'n}$.

\label{sec:inducedkernel}
Our analysis will rely heavily on nonlinear random matrix theory. These nonlinear random matrices will come principally in two forms: (1) random kernel matrices, whose general entry is of the form $\kappa(a_i^\top a_j)$ for iid random vectors $a_1,a,\ldots$ on a finite-dimensional vector space (e. $\mathbb R^d$ or $\mathbb R^k$), and (2) random feature design matrices whose entries are of the form $h(a_i^\top b_j)$, for some nonlinear function $h:\mathbb R \to \mathbb R$, and random vectors $a_1,b_1,a,b,\ldots$ on a finite-dimensional vector space. For the first scenario, will use classical RMT tools from \cite{elkaroui2010}, whilst for the second scenario, we will the \emph{free probabilistic} results from ~\cite{pennington17,peche19,Hastie2019}.

\subsection{Kernels induced by homogeneous activation functions}
% We start with some preliminaries.
\begin{restatable}[Induced kernel function]{df}{}
Given a measurable function $h:\mathbb R \to \mathbb R$, define the kernel function $K_h:\sphere \times \sphere \to \mathbb R$ by
\begin{equation}
    K_h(a,b) := \mathbb E_x[h(x^\top a)h(x^\top b)],
\end{equation}
for $x \sim \tau_d$ (i.e uniformly random on the unit-sphere $\sphere$).
\label{df:kernelfunc}
\end{restatable}
% A subclass of kernel functions will be particularly important to us.

Now, for $a,b \in \sphere$, let $\angle(a,b) \in [0, \pi]$ be their angle, defined by
\begin{eqnarray}
\begin{split}
\angle(a,b) &:=\arccos(a^\top b).
\end{split}
\end{eqnarray}
The following proposition will be very helpful in the sequel.
\begin{restatable}[Kernel function induced by homogeneous activations
~\cite{Erez2016}]{prop}{}
\label{prop:catalan}
If $h:\mathbb R \to \mathbb R$ is positive-homogeneous of order $p \ge 0$, then for every $a,b \in \sphere$ we have the identity
\begin{equation}
    K_h(a,b)=\kappa_h(a^\top b),\text{ with }\kappa_h(u) := \dfrac{C_{2,2p}}{2\pi C_{d,2p}}\int_{0}^{2\pi}h(\cos t)h(\cos(t-\arccos u))\dif t,
\end{equation}
where $C_{d,p} := 2^{p/2-1}\cdot \dfrac{d\cdot \Gamma((d+p)/2)}{\Gamma((d+2)/2)}$.
\end{restatable}
Thus, positive-homogeneous activation functions induce kernel functions of dot-product type (aka dot-product kernels).
\subsection{Sobolev-seminorm of homogeneous two-layer neural networks}
\label{sec:sob}
For any two-layer neural network $f=f_{W,v} \in \mathcal F_{d,k}(\sigma)$, the squared Sobolev-seminorm $\mathfrak{S}(f)^2$ of $f$ w.r.t $x \sim \tau_d$ writes
\begin{eqnarray}
\begin{split}
\mathfrak{S}(f)^2 := \mathbb E_x \|\nabla_{\sphere} f(x)\|^2 &= \mathbb E_x\|\nabla f(x)\|^2 - \mathbb E_x (x^\top \nabla f(x))^2\\
 &= \mathbb E_x \|\nabla f(x)\|^2 - p\mathbb E_x [|f(x)|^2],
\end{split}
\end{eqnarray}
% Now, by Cauchy-Schwarz, $\mathbb E_x (x^\top \nabla f(x))^2 \le \mathbb E_x \|x\|^2\|\nabla f(x)\|^2$
where we have used the order-$p$ positive-homogeneity of the activation function $\sigma$ in the last step (\emph{Euler's Theorem}). We now compute each term of the rightmost side separately.

\emph{The first term.} Now, $f(x) := v^\top\sigma(Wx) = \sum_{j=1}^k v_j\sigma(x^\top w_j)$ and so
\begin{eqnarray*}
\begin{split}
\mathbb E_x \|\nabla f(x)\|^2 &= \mathbb E_x \|\sum_{j=1}^kv_j\sigma'(x^\top w_j)w_j\|^2 = \mathbb E_x\sum_{j=1}^k\sum_{\ell=1}^kv_jv_\ell\sigma'(x^\top w_j)\sigma'(x^\top w_\ell)w_j^\top w_\ell\\
&=\sum_{j=1}^k\sum_{\ell=1}^kv_jv_\ell \mathbb E_x[\sigma'(x^\top w_j)\sigma'(x^\top w_\ell)]w_j^\top w_\ell = \|v\|^2_{ K_{\sigma'}(W) \circ WW^\top},
\end{split}
\end{eqnarray*}
where $K_{\sigma'}(W)$ is the $k \times k$ matrix with entries $(K_{\sigma'})_{j,\ell} := K_\sigma'(w_j,w_\ell)$ and $K_{\sigma'}:\sphere \times \sphere \to \mathbb R$ is the kernel function induced by the derivative $\sigma'$ of $\sigma$ (see Definition \ref{df:kernelfunc}).
%where the kernel function $\kappa_{\sigma'}:\mathbb R^d \times \mathbb R^d \to \mathbb R$ is defined by
%\begin{equation}
%K_{\sigma'}(a,b) := \mathbb E_x [\sigma'(x^\top a)\sigma'(x^\top b)]. % \end{equation}
% For example, if $\sigma(t) := \max(t,0)$, then $K_{\sigma'}(a,b) :=  \dfrac{\arccos(-t(a,b))}{2\pi}$.

\emph{The second term.} One computes $|f(x)|^2 = \sum_{j=1}^k \sum_{\ell=1}^k v_jv_\ell \sigma(x^\top w_j)\sigma(x^\top w_\ell)$, and so
$$
\mathbb E_x [f(x)^2] = \sum_{\ell=1}^k v_jv_\ell\mathbb E_x[\sigma(x^\top w_j)\sigma(x^\top w_\ell)] = \|v\|^2_{K_{\sigma}(W)}.
$$
% where $K_\sigma(a,b) := \mathbb E_x[\sigma(x^\top a)\sigma(x^\top b)]$, for all $a,b \in \mathbb R^d$. In particular, if $\sigma=\text{ReLU}$, then $K_\sigma(a,b) = \|a\|\|b\|\left(\dfrac{t \arccos(-t(a,b))+\sqrt{1-t(a,b)^2}}{2\pi d}\right)$.

Let $C_\sigma(W)=K_{\sigma'}(W) \circ WW^\top - pK_\sigma(W)$ be the $k \times k$ psd matrix with entries
\begin{eqnarray}
\label{eq:analytic}
C(w_j,w_\ell) := w_j^\top w_\ell K_{\sigma'}(w_j,w_\ell)-pK_{\sigma}(w_j,w_\ell)\;\forall j,\ell \in [k].
\end{eqnarray}
Putting things together, we obtain the following result which will be an important corner stone in most of the remainder of the analyses.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Analytic formula for Sobolev norm of two-layer neural network]{thm}{}
For any $f=f_{W,v} \in \mathcal F_{d,k}(\sigma)$, we have the identity
\begin{eqnarray}
\mathfrak{S}(f)^2 = v^\top C_\sigma(W)v.
\end{eqnarray}
\label{thm:analytic}
\end{restatable}
\end{mdframed}
Thanks to the definition of extreme singular-values of matrices, we know that
\begin{eqnarray}
\label{eq:sandwitch}
\lambda_{\min}(C_\sigma(W))\|v\|^2 \le \|v\|^2_{C_\sigma(W)} \le \lambda_{\max}(C_\sigma(W))\|v\|^2.
\end{eqnarray}
Thus in virtue of Theorem \ref{thm:analytic}, to get lower- and upper-bounds for the robustness $\mathfrak{S}(f)$, it suffices to control the extreme singular-values of $C_\sigma(W)$. The great deal of the analysis in the rest of the manuscript will indeed be about controlling the extreme values of $C_\sigma(W)$ (and analogous matrices derived from applying Poincar\'e's inequality), under different regimes (random features, NTK, etc.).

% In the following section we will exploit the above identity to estimate the robustness of models in $\mathcal F_{,k}(\sigma)$ which minimize generic data $\mathcal D_n$.

\subsection{Simplifying the kernel matrix $C_\sigma(W)$}
Note that since $\sigma$ is is positive-homoegeneous of order $p \ge 1$, it follows that it's derivative $\sigma'$ is positive-homoegeneous of order $p-1$. By Proposition \ref{prop:catalan}, the induced kernel functions $K_\sigma$ and $K_{\sigma'}$ are of dot-product type.
Let $\kappa_{\sigma'},\kappa_\sigma:\mathbb R \to \mathbb R$ be functions such that $K_{\sigma'}(a,b) = \kappa_{\sigma'}(a^\top b)$ and $K_\sigma(a,b)=\kappa_\sigma(a^\top b)$ for all $a,b \in \sphere$.
% % , the existence of which is guaranteed by Proposition \ref{prop:catalan}.
% Define
$\widetilde{\kappa}_\sigma:[-1,1] \to \mathbb R$ by
\begin{eqnarray}
\label{eq:badrho}
\widetilde{\kappa}_\sigma(t) := t\kappa_{\sigma'}(t) - p\kappa_{\sigma}(t).
\end{eqnarray}
We can then rewrite the kernel $C_\sigma(W)$ appearing in Theorem \ref{thm:analytic} as \begin{eqnarray}
(C_\sigma(W))_{j,\ell} = \widetilde{\kappa}_\sigma(w_j^\top w_\ell),\;\text{ for all }j,\ell \in [k].
\label{eq:simpleanalytic}
\end{eqnarray}
The scalar function $\widetilde{\kappa}_\sigma$ is depicted in Table \ref{tab:maclaurin} for variance activation functions.

% It turns out that the function $\widetilde{\kappa}_\sigma$ in \eqref{eq:simpleanalytic} is dominated by the first part $\kappa_{\sigma'}$.
% Indeed,
% \begin{restatable}{lm}{}
% We have the approximation
% $\|\widetilde{\kappa}_\sigma-\kappa_{\sigma'}\|_\infty = \mathcal O(1/d)$.
% \end{restatable}
% \begin{proof}
% Indeed, let $t \in [-1,1]$ and $u,v \in \sphere$ such that $u^\top v = t$. One computes
% \begin{eqnarray*}
% \begin{split}
% |\widetilde{\kappa}_\sigma(t)-\kappa_{\sigma'}(t)|^2= |\kappa_\sigma(t)|^2 =|\mathbb E_x[\sigma(x^\top u)\sigma(x^\top v)]|^2 &= |\mathbb E_x[(x^\top u)(x^\top v)\sigma'(x^\top u)\sigma'(x^\top v)]|^2\\
% &\le C\mathbb E_x[(x^\top u)^2(x^\top v)^2] = \mathcal O(\frac{1}{d^2}),
% \end{split}
% \end{eqnarray*}
% where we have used the Cauchy-Schwarz inequality and the fact that $\|\sigma'\|_\infty \le C < \infty$ since $\sigma'$ is a.e continuous, and positive-homogeneneous of order $1-1=0$.
% \end{proof}
% The function $\widetilde{\kappa}_\sigma$ will be central in our analysis of the (non)robust memorization properties of functions in $\mathcal F_{d,k}(\sigma)$.
\begin{table}[h!]
  \begin{center}
       {\tabulinesep=1.2mm
    \begin{tabu}{|c|c|c|}
    \hline
       $\sigma$ & $\widetilde{\kappa}_\sigma(t):=t\kappa_{\sigma'}(t)-\kappa_\sigma(t)$ & Maclaurin expansion of $\widetilde{\kappa}_\sigma$ \\
      \hline
        ReLU & $\dfrac{t\arccos(-t)}{2\pi}-\dfrac{t\arccos(-t)+\sqrt{1-t^2}}{2\pi d}$ &
        $\dfrac{1}{4}t+\dfrac{1}{2\pi}t^2+\mathcal O(t^3,\dfrac{1}{d})$\\
      \hline
        Absolute value & $\dfrac{2t\arcsin(t)}{\pi}-\dfrac{2t\arcsin(t)+2\sqrt{1-t^2}}{\pi d}$ & $\dfrac{2}{\pi}t^2+\mathcal O(t^3,\dfrac{1}{d})$\\
      \hline
    \end{tabu}
    }
  \end{center}
    \caption{Table of the function $\widetilde{\kappa}_\sigma$ for a variety of popular activation functions $\sigma$.}
\label{tab:maclaurin}
\end{table}
% \lorem

% \section{Random features regime with homogeneous activation functions}
% \label{sec:rfhom}
% Consider an order-$1$ positive-homogeneous activation function and let $\widehat{f}_{\rf} \in \mathcal F_{d,k}(\sigma)$ be the random features model with random hidden weights matrix $W=(w_1,\ldots,w_k) \in \mathbb R^{k \times d}$ for iid $w_1,\ldots,w_k \sim \tau_d$, and output weights vector $v \in \mathbb R^k$ is fitted on generic dataset $\mathcal D_n$,
% % = \{(x_1,y_1),\ldots,(x_n,y_n)\}$ (see section \ref{sec:prelim} for definition of generic dataset),
% i.e $v$ is the least-squares solution to the linear system of equations $v^\top z_i = y_i$ for all $i \in [n]$, where $Z=(z_1,\ldots,z_n)$ is the $n \times k$ random matrix with entries $z_{i,j} := \sigma(x_i^\top w_j)$.
% Our results can be readily extended to positive-homogeneous function.

% We will linearize the kernel random matrix $C_\sigma(W)$, and consistently approximate its entire spectrum with that of a spiked Wishart covariance model $\alpha \mathbbm 1_k\mathbbm 1_k^\top + \beta WW^\top + \gamma I_k$, where $\alpha$, $\beta$, and $\gamma$ are scalars which only depend on the activation function (and perhaps the input dimension $d$). See Lemma \ref{lm:specC}. Equipped with this linearization, we will prove there that w.p $1-d^{-1+o(1)}$ over the choice of $W$, the following hold
% \begin{itemize}
% \item (Corollaries \ref{cor:Cspecrelu} and \eqref{cor:Cspecrelulike}) The eigenvalues of kernel random matrix $C_\sigma(W)$ defined in \eqref{eq:analytic} are contained in a compact interval $[c_1,c_2]$, where $c_1,c_2>0$ are absolute constants.
% \item (Theorem \ref{thm:relusob}) $\Lip_{\sphere}(f_{W,v}) \ge\mathfrak{S}(f_{W,v}) = \Theta(\|v\|)$ for any $v \in \mathbb R^k$.
% \end{itemize}
% The second result is a direct consequence of the first, combined with Theorem \ref{thm:analytic}. Thus, in such random features regimes, the $L_2$-norm of the output weights vector completely characterizes its (non)robustness!
% Thus, we have identified a new regime for Conjecture \ref{conj:bubeck}, in which the predicted nonrobustness is quadratically much worst!

% \begin{restatable}{rmk}{}
% Comparing Corollary \ref{cor:Cspecrelu} and \ref{cor:Cspecquad}, we see a gap in the nonrobustness lower-bounds, between the ReLU and the quadratic activation function in the over-complete case where $d>k$. Indeed, in this scenario it holds w.p $1-d^{-\Omega(1)}$ over the choice of $W$ that
% \begin{itemize}
%     \item[--] ReLU activation function: $\mathfrak{S}(f_{W,v})=\Theta(\|v\|)$, and
%     \item[--] Quadratic activation function: $\Omega (\|v\|/\sqrt{k}) \le \mathfrak{S}(f_{W,v}) \le \mathcal O(\|v\|)$.
% \end{itemize}
% So while in the case of ReLU activation all bets are off, in the case of the quadratic activation there is hope that over-parametrization might reduce the nonrobustness of the model.
% \end{restatable}

% \subsection{Nonrobust memorization in infinite-width random features regime}
% We now consider the random features regime with $n,d,k \to \infty$ according to the proportional scaling \eqref{eq:proportionate}. Define $Z := \sigma(XW^\top) \in \mathbb R^{n \times k}$.
% % Thanks to the approximation \eqref{eq:linearize}, we know that nonlinear random $k \times k$ gram matrix $Z^\top Z$ is invertible almost-surely. Thus
% For a ridge regularization parameter $\lambda > 0$, the optimal output weights of the random features model are given by $\widehat{v}_\lambda = (Z^\top Z + n\lambda I_k)^{-1}Z^\top y \in \mathbb R^k$.

% \subsection{Proof of Theorem \ref{thm:law}}
% For a regularization parameter $\lambda > 0$, consider a random features model $\widehat{f}_{\rf,\lambda}:x \mapsto \widehat{v}_\rf(\lambda)^\top \sigma(Wx)$ obtained by solving the following ridge-regression problem for the output weights
% \begin{eqnarray}
% \label{eq:genprob}
% \arg\min_{v \in \mathbb R^k}\frac{1}{n}\sum_{i=1}^n(y_i-v^\top \sigma(Wx_i))^2 + \frac{k\lambda}{d}\|v\|^2.
% \end{eqnarray}
% Note that we have the explicit formula $\widehat{v}_\rf(\lambda) =(ZZ^\top/n + \lambda(k/d) I_n)^{-1}Z^\top y$ for any $\lambda>0$.
% % Removing this restriction is left for future work.
% Since we are considering positive-homogeneous functions, the above condition is automatically satisfied.

% \law*
% The prediction of theorem is empirically confirmed in Figure \ref{fig:peaks}.
%  \begin{figure}
%     \centering
%     % \includegraphics[width=.48\linewidth]{law.png}
%     \includegraphics[width=.48\linewidth]{rf_infinite_width_big=False=True.png}
%     \caption{Law of robustness for random features model in proportional scaling regime. Here the activation function is the ReLU. Each color corresponds to experiments with $\gamma$ in the given range. Each point corresponds to a different value of the triple $(n,d,k)$, and draws of the random dataset $\mathcal D_n$ and also of the hidden weights matrix $W$ of the network.}
%     \label{fig:my_label}
% \end{figure}

% Decompose the activation function $\sigma$ as $\sigma(x) = \mu_0 + \mu_1x + \sigma_\perp(x)$ where $\mathbb E[\sigma_\perp(z)] = \mathbb E[z\sigma_\perp(z)] = 0$ for $z \sim N(0,1)$. A simple calculation reveals that such a decomposition is uniquely obtained by setting $\mu_0 := \mathbb E[\sigma(z)]$ and $\mu_1 := \mathbb E[z\sigma(z)]$. Now, define $\mu_\star \ge 0$ by $\mu_\star^2 := \mathbb E[\sigma_\perp(z)^2]$. Note that $\mu_\star = 0$ iff the activation function $\sigma$ is affine. Otherwise, the linearization of the nonlinear random gram matrix $Z^\top Z$ is spiked Wishart matrix
% \begin{eqnarray}
% \begin{split}
% Z^\top Z &= \mu_0^2 1_k1_k^\top + \mu_1^2 WW^\top + \mu_\star^2 I_k + \Delta,% \\
% % Z Z^\top &= \mu_0^2 1_d 1_d^\top + \mu_1^2 W^\top W + \mu_\star^2 I_d + \Delta'.
% \end{split}
% \label{eq:linearize}
% \end{eqnarray}
% where $\|\Delta\|_{op} = o_{\mathbb P}(1)$. A few examples (ReLU activation, identity, power, etc.) are depicted in Table \ref{Tab:linearize}.
% \begin{table}[h!]
% \label{tab:maclaurin}
%   \begin{center}
%       {\tabulinesep=1.2mm
%     \begin{tabu}{|c|c|c|c|}
%     \hline
%       Activation function $\sigma$ & $\mu_0^2$ & $\mu_1^2$ & $\mu_\star^2$\\
%       \hline
%       Indentity $\sigma(x):=x$ & $0$ & $1$ & $0$\\
%       \hline
%       ReLU $\sigma(x):=x \lor 0$ & $\dfrac{1}{2\pi}$ & $\dfrac{1}{4}$ & $\dfrac{\pi-2}{4\pi}=\Omega(1)$\\
%     \hline
%       Power $\sigma(x):=x^p$, $p$ even & $\nu_p$ & $0$ & $\nu_{2p}-\nu_p^2=\Omega(1)$\\
%     \hline
%     \end{tabu}
%     }
%   \end{center}
%     \caption{(Refer to \eqref{eq:linearize}) Linearization parameters for nonlinear gram matrices associated to different activation functions. Note that $\nu_p$ is the $p$th moment of the standard normal distribution $N(0,1)$.}
%     \label{Tab:linearize}
% \end{table}

% \lorem
% For the proof, we will need the following lemma.
% \begin{restatable}{lm}{}
% Under the hypotheses of Theorem \ref{thm:nonrobRF}, in-sample mean squared error of $\widehat{f}_{\rf}$ verifies
% \begin{eqnarray}
% \mathrm{MSE}(\widehat{f}_{\mathrm{RF}}):= \frac{1}{n}\sum_{i=1}^n (y_i - \widehat{f}_{\rf}(x_i))^2=(1-\frac{1}{\gamma})_+ + o_{\mathbb P}(1).
% \label{eq:gammafit}
% \end{eqnarray}
% Thus $\widehat{f}_{\rf}$ memorizes generic data $\mathcal D_n$ with probability tending to $1$.
% \label{lm:gammafit}
% \end{restatable}
% The above lemma is not new, at least it appears ~\cite{pennington17} in the weaker form $\mathbb E_y \mathrm{MSE}(\widehat{f}_{\rf}) = (1-1/\gamma)_+$. Here, we provide the a $\mathcal O(1/n)$ upper-bound for the variance (which is valid outside a small bad event).
% \begin{proof}[Proof of Lemma \ref{lm:gammafit}]
% Since the rows of $Z$ have density w.r.t Lebesgue, $Z$ has full rank $n \land k$, on an event $\mathcal E_n$  with $\mathbb P(\mathcal E_n) =1-o(1) \to 1$.
% Now, the in-sample mean squared error (MSE) of $\hat{f}_{\mathrm{RF}}$ writes
% $$
% R_n  := \frac{1}{n}\|y-Z\widehat{v}\|^2 = \frac{1}{n}\|(I-ZZ^\dagger)y\|^2 = 1 - \frac{1}{n}\|P_{\Image(Z)}y\|^2,
% $$
% where $Z^\dagger$ is the Moore-Penrose pseudo-inverse of $Z$ and $P_{\Image(Z)} \in \mathbb R^n$ is the orthogonal projector onto the the subspace spanned by the rows of $Z$.
% One then computes the expectation of the in-sample MSE conditioned on the event $\mathcal E_n$ as
% $$
% \mathbb E[R_n \mid \mathcal E_n] = 1-\dfrac{1}{n}\trace(P_{\Image(Z)}) = 1-\dfrac{\rank(Z)}{n} = 1-\dfrac{n \land k}{n}=(1-\dfrac{1}{\gamma})_+,
% $$
% and the variance thereof as
% \begin{eqnarray*}
% \begin{split}
% \var[R_n \mid \mathcal E_n] &= \frac{2}{n^2}\trace(P_{\Image(Z)}^2) = \frac{2}{n^2}\trace(P_{\Image(Z)})= \frac{2}{n^2}\rank(Z) = \frac{n\land k}{n^2} = \frac{1}{(\gamma \land 1)n}=\mathcal O(\frac{1}{n}).
% \end{split}
% \end{eqnarray*}
% Setting $r:=\mathbb E[R_n \mid \mathcal E_n] = (1-1/\gamma)_+$, one computes for every $t > 0$,
% \begin{eqnarray*}
% \begin{split}
% \mathbb P(|R_n-r| \le t) &= \mathbb P(|R_n-\mathbb E[R_n \mid \mathcal E_n] \le t)\\
% &\ge \mathbb P(\mathcal E_n)\mathbb P(|R_n - \mathbb E[R_n \mid \mathcal E_n] \le t \mid \mathcal E_n) \\
% &\ge \mathbb P(\mathcal E_n)(1-\frac{\var(R_n \mid \mathcal E_n)}{t^2})\\
% &= \mathbb P(\mathcal E_n)(1-\mathcal O(\frac{1}{t^2n}))\\
% &= (1-o(1))(1-\mathcal O(\frac{1}{t^2n})) \to 1,
% \end{split}
% \end{eqnarray*}
% where the second inquality is an application of Chebychev's ienquality. We conclude that $R_n=(1-1/\gamma)_+ + o_{\mathbb P}(1)$ as claimed.
% \end{proof}

% \lorem

% \begin{restatable}{lm}{} Let $\zeta$ be a random vector in $\mathbb R^m$ with zero mean and identity covariance matrix and let $A$ be a symmetric $m \times m$ random matrix independent of $\zeta$. Then
% \begin{eqnarray}
% \begin{split}
% \mathbb E[y^\top A y] &= \mathbb E[\trace(A)],\text{ and}\\
% \mathbb E[(y^\top A y)^2] &= 2\mathbb E[\trace(A^2)] + \mathbb E[\trace(A)^2].
% \end{split}
% \end{eqnarray}
% \end{restatable}
% \begin{proof}
% By the standard formula for the expectation of a quadratic form, we have
% $$
% \mathbb E[y^\top A y] = \mathbb E_A\mathbb E_{y \mid A}[y^\top A y] = \mathbb E_A[\trace(A\cov(y))] = \mathbb E[\trace(A)].
% $$
% On the other hand, using the \emph{law of total variance},
% \begin{eqnarray*}
% \begin{split}
% \mathbb E[(y^\top A y)^2] &= \var(y^\top A y)+(\mathbb E[(y^\top A y)])^2\\
% &= 2\mathbb E[\trace(A^2)] + \var(\trace(A)) + (\mathbb E[(y^\top A y)])^2\\
% &= 2\mathbb E[\trace(A^2)] + \var(\trace(A)) + (\mathbb E[\trace(A)])^2\\
% &= 2\mathbb E[\trace(A^2)] + \mathbb E[\trace(A)^2],
% \end{split}
% \end{eqnarray*}
% which completes the proof.
% \end{proof}

% \begin{proof}[Proof of Theorem \ref{thm:nonrobRF}]
% % The first part is a direct consequence of ~\cite{pennington17,peche19,Hastie2019}. Indeed, we can deduce from their results that the mean squared error of $\widehat{f}_{\rf}$ on the dataset $\mathcal D_n$ converges to $(1-k/n)_+$ in probability. To prove the second part, we only need lower-bound the norm of the output weights vector $\|v\|$ and then invoke Corollary \ref{thm:relusob} with the crucial condition that $k=\Theta(d)$. Since $k/n = \lambda \in (0,1)$ by assumption, the random features matrix $Z$ is full-rank a.s \mytodo{ This looks like bs; cite references and exact statements!} and so
% The output weights vector of $\widehat{f}_{\rf}$ is $\widehat{v} = Z^\dagger y$, where $Z:=\sigma(XW^\top)$ is the $n \times k$ matrix with entries given by $z_{ij} := \sigma(x_i^\top w_j)$ and $Z^\dagger$ is the Moore-Penrose pseudo-inverse of $Z$.
% Let $P^\perp := I_n-ZZ^\dagger$ be orthogonal projection onto the null-space of $Z$. Note that $P^\perp$ has rank $n-\rank(Z)$, and so the empirical in-sample error of $\widehat{f}_{\rf}$ writes
% $$
% \frac{1}{n}\|y-Z\widehat{v}\|^2=\frac{1}{n}\|P^\perp y\|^2 = \frac{1}{n}(n-\rank(Z)) = 1-\frac{\rank(Z)}{n}.
% $$
% We conclude that if $Z$ is full rank (i.e if $\rank(Z) = \min(n,k))$, then $\widehat{f}_{\rf}$ memorizes the dataset $\mathcal D_n$ (in the sense of  definition \ref{df:memo}). We will eventually prove that $Z$ is indeed full-rank w.h.p, but for now let us lower-bound $\|\widehat{v}\|$.

% Now, the Paley-Zygmund inequality tells us that for all $\theta \in (0,1)$,
% \begin{eqnarray}
% \label{eq:pz}
% \mathbb P(\mathbb [\|\widehat{v}\|^2 \ge \theta\mathbb E[\|\widehat{v}\|^2]) \ge (1-\theta)^2 \frac{(\mathbb E[\|\widehat{v}\|^2])^2}{\mathbb E[\|\widehat{v}\|^4]}.
% \end{eqnarray}
% Let $A := (Z^\dagger)^\top Z^\dagger$ (a random $n \times n$ psd matrix), so that $\|\widehat{v}\|^2 = y^\top A y$, a quadratic form in $y$, with coefficient matrix $A$. By standard formulae for moments of random quadratic forms, we obtain
% \begin{eqnarray}
% \begin{split}
% \mathbb E[\|\widehat{v}\|^2] &= \mathbb E [y^T A y] = \mathbb E[\trace(A)], \text{ and }\\
% \var(\|\widehat{v}\|^2)& =2\mathbb E[\trace(A^2)]+\mathbb E[\trace(A)^2].
% \end{split}
% \end{eqnarray}
% Plugging all of this in \eqref{eq:pz} and setting $\eta(A) := \trace(A)^2/\trace(A^2) \ge 1$, we obtain that $\forall \theta \in (0, 1)$,
% $$
% \mathbb P(\|\widehat{v}\|^2 \ge \theta \trace(A) \mid X, W) \ge (1-\theta)^2\frac{1}{1+2/\eta(A)} \ge \frac{(1-\theta)^2}{3}.
% $$
% It is clear that both $\trace(A)$ and $\eta(A)$ depend on $A:=(Z^\dagger)^\top Z$ only via the singular-values $s_1(Z) \ge s(Z) \ge \ldots \ge s_{\mathrm{rank}(Z)}(Z)$ of $Z$. Indeed, it is easy to see that for any nonnegative integer $m$,
% $$
% \trace(A^m) = \sum_{i=1}^{\mathrm{rank}(Z)}s_i(Z)^{-2m}=\sum_{i=1}^{\mathrm{rank}(Z)}s_i(Z^\top Z)^{-m}.
% $$
% % where we have used the elementary fact that $\trace(A^m) = \trace(Q^m)$ for every nonnegative integer $m$.
% % Letting $n,k \to \infty$ (again, with $k/n = \lambda$) gives
% \begin{eqnarray}
% \begin{split}
% % \|\widehat{v}\|^2 = \trace(\widehat{v}\widehat{v}^\top) = \trace(Q Z^\top yy^\top Z Q)\overset{p}{\longrightarrow} \trace(Q Z^\top Z Q) = \trace(Q^2 Z^\top Z)=\trace(Q),
% \|\widehat{v}\|^2 = \|QZ^\top y\|^2 \ge \|y\|^2\cdot \lambda_{\min}(QZ^\top Z Q) = n\lambda_{\min}(Q).
% \end{split}
% \label{eq:trace}
% \end{eqnarray}

% % where we have used the fact that $yy^\top \to I_n$ in probability.
% But thanks to ~\cite{pennington17,peche19,Hastie2019} again, $Z^\top Z$ has a limiting distribution which is Marchenko-Pastur distribution with parameter $\lambda/2$. Thus in particular, $\lambda_{\min}(Q) = \Omega_{\mathbb P}(1)$
% % the eigenvalues are asymptotically contained in $[(1-\sqrt{\lambda})^2,(1+\sqrt{\lambda})^2]$. We deduce that $\|\widehat{v}\|^2 = \trace(Q) \overset{p}{\longrightarrow} \sum_{i=1}^n \dfrac{1}{\lambda_i(Z^\top Z)} =\Theta_{\mathbb P}(n)$ 
% and combining with Theorem \ref{thm:relusob} then gives the result.
% \end{proof}

% \input{rf_linear_interp.tex}

==> general.tex <==
\begin{restatable}[Spectral ratio]{df}{}
Given $W \in \mathbb R^{k \times d}$, define its spectral ratio relative to the activation function $\psi$, denoted $\condnumb_\psi^{-1}(W)$, by
\begin{eqnarray}
\condnumb_\psi^{-1}(W):= \sqrt{\dfrac{\lambda_{\min}(C_\psi(W))}{\lambda_{\max}(WW^\top)}},
\label{eq:cond}
\end{eqnarray}
and $C_\psi(W) \in \mathbb R^{k \times k}$ is the covariance matrix of defined in \eqref{eq:C}.
\end{restatable}

\paragraph{Link with condition number (linear algebra).}
Observe that linear models correspond to taking $\psi = \psi_\text{id}$, the identity activation function defined by $\psi_{\text{id}}(t) = t$ for all $t \in \mathbb R$. A direct computation then yields $C_{\psi_{\text{id}}}(W) = d(W(1/d)I_dW^\top=WW^\top $, from which we deduce that
\begin{eqnarray}
\condnumb_{\psi_{\text{id}}}^{-1}(W) = \sqrt{\dfrac{\lambda_{\min}(WW^\top )}{\lambda_{\max}(WW^\top)}} = \dfrac{1}{\condnumb(W)},
\label{eq:condlinalg}
\end{eqnarray}
where $\condnumb(W) := \|W\|_{op}\|W^\dagger\|_{op}$ is the \emph{condition number} of $W$, i.e the ratio of the largest to smallest singular-value of $W$. 


\subsection{Template bound for general regime}
The following theorem is one of our main results, and provides a generic path to solving Conjecture \ref{conj:bubeck}, via the spectral of $WW^\top$ and the kernel matrix $C_\psi(W)$. Viz,
% \mytodo{Consider approximate fit: $\#\{i \in [\![n]\!] \mid v^\top \psi(Wx_i)=y_i\} \ge n$.}
%\mytodo{It turns out that we consider leaky ReLU activations form (17) or \url{https://papers.nips.cc/paper/2017/file/0f3d014eead934bbdbacb62a01dc4831-Paper.pdf}} 
%Let $\psi:\mathbb R \to \mathbb R$ be a continuously differentiable a.e, and consider two-layer neural networks $f$ as defined in \eqref{eq:tlnn}.

% \subsection{Non-robustness of random features regime}
% \label{sec:rf}
% Suppose $W$ is initialized with random iid entries from $\mathcal N(0,s^2/d)$, where $s \in (0, 1]$ is a scaling parameter for the weights.

% \begin{restatable}[Norm of output layer weights is large!]{thm}{}
% It holds with $1-o(1)$ over generic data $(x_1,y_1),\ldots,(x_n,y_n)$ and the choice of hidden weights $w_1,\ldots,w_k \overset{iid}{\sim} \mathcal N(0,(1/d)I_d)$, that the $L_2$-norm of any choice of $v \in \mathbb R^k$ of outputs weights which fits the data satisfies
% \begin{eqnarray}
% \|v\| \ge C\sqrt{\frac{nd}{k}} \cdot \begin{cases}1,&\mbox{ if }\psi=\mathrm{id},\\n^{-o(1)},&\mbox{ if }\psi=\mathrm{ReLU},\\n^{-o(1)}\sqrt{d},&\mbox{ if }\psi=\mathrm{quadratic.}
% \end{cases}
% \label{eq:vnorm}
% \end{eqnarray}
% \label{thm:vnorm}
% \end{restatable}
% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=\linewidth]{lor.png}
%     \caption{Empirical validation of Theorem \ref{thm:vnorm}, in the setting $k \asymp n$. Error-bars represent different draws of the parameters of each neuron from $\mathcal N(0,1/d)$. As predicted by the theorem, we see that $\|v\| = \Omega(\sqrt{d})$ (i.e linear in $\sqrt{d}$) for ReLU activations, and $\|v\|=\Omega(d)$ (i.e quadratic in $\sqrt{d}$) for the quadratic activation function.}
%     \label{fig:my_label}
% \end{figure}
% \begin{proof}
% Let $\overline{z} := \sum_{i=1}^n y_i \psi(Wx_i)$. A direct computation gives
% $$
% \overline{z}^\top v = \sum_{i=1}^n y_i \psi(Wx_i)^\top v = \sum_{i=1}^n y_i^2 = n,
% $$
% and so Cauchy-Schwarz yields
% \begin{eqnarray}
% \|v\| \ge \frac{n}{\|\overline{z}\|}.
% \label{eq:cs}
% \end{eqnarray}
% The rest of the prove is about lower-bounding $\|\overline{z}\|$ and plugging into the above inequality.

% \paragraph{-- Step 1: Covering argument.} Note that $\|\overline{z}\| = \max_{\|u\| = 1}u^\top\overline{z}$.
% Let $\mathcal C_\epsilon = \{u_1,\ldots,u_{N_\epsilon}\} \subseteq \mathbb R^k$ be an cover for the $(k-1)$-dimensional unit-sphere $\mathbb S_{k-1}$, with $N_\epsilon \le (1/\epsilon)^k$. For any $u \in \mathbb S_{k-1}$, there exists $u_\epsilon \in \mathcal C_\epsilon$ such that $\|u-u_\epsilon\| \le \epsilon$. A simple covering argument gives
% $$
% \|\overline{z}\| = \sup_{\|u\| = 1}u^\top\overline{z} \le \sup_{\|u\| = 1} u^\top\overline{z}_\epsilon + \epsilon \|\overline{z}\| \le \sup_{u \in \mathcal C_\epsilon}u^\top\overline{z} + \epsilon\|\overline{z}\|.
% $$
% Taking $\epsilon=1/2$, we obtain
% \begin{eqnarray}
% \|\overline{z}\| \le 2\sup_{u \in \mathcal C_{1/2}}u^\top\overline{z}.
% \label{eq:tag1}
% \end{eqnarray}

% \paragraph{-- Step 2: Concentration.} Let $r$ be the RHS of \eqref{eq:vnorm}. For any unit-vector $u \in \mathbb S_{k-1}$, we know from Lemma \ref{lm:nonlip} that $\mathbb P(|u^\top\overline{z}| \ge r \mid \mathscr F_n) = e^{-Ck}$, where
% \begin{itemize}
% \item $\mathscr F_n$ is an event which only depends on the data (i.e is independent of the $w_j$'s) and occurs with probability $1-e^{-\Omega(d \land \tau})$, and
% \item $C>0$ is a constant which can be chosen so that $2^ke^{-Ck} = e^{-\Omega(k)}$.
% \end{itemize}
% Taking $\tau = n^{2\delta}$ for small $\delta > 0$, conditioning on $\mathscr F_n$, and applying a union-bound, we have
% $$
% \mathbb P(\sup_{u \in \mathcal C_{1/2}} u^\top\overline{z} \ge r \mid \mathscr F_n) \le N_{1/2} \cdot e^{-Ck} \le \mathcal O(2^k) \cdot e^{-Ck} = e^{-\Omega(k)},
% $$
% It then follows from \eqref{eq:tag1} that
% $$
% \mathbb P(\|\overline{z}\| \le r \mid \mathscr F_n) \ge 1-e^{-\Omega(k)}.
% $$
% Combining with \eqref{eq:cs}, we obtain that $\|v\| \ge \Omega(r)$ w.p at least
% $$
% (1-\mathbb P(\mathscr F_n))e^{-\Omega(k)}=(1-e^{-\Omega(\sqrt{n} \land \tau)})(1-e^{-\Omega(k)}) = 1-e^{-\Omega(d \land \tau \land k)}=1-o(1),
% $$
% which completes the proof.
% \end{proof}

% \begin{restatable}{lm}{nonlip}
% Let $0 < \tau \le n$ and define $\mathscr F_n$ to be the event that (A) $\|X\|_{op} = \mathcal O(1)$, and (B) $|\sum_{i=1}^n y_i| \le \sqrt{n\tau}$.
% Then $\mathbb P(\mathscr F_n) \ge 1 - o(1)$, and if we take $\tau : = n^{2\delta}$ for small $\delta > 0$ and let $r$ be the RHS of \eqref{eq:vnorm}, then $\mathbb P(|u^\top\overline{z}| \ge nr \mid \mathscr F_n) \le 2\exp(-\Omega(k))$.
% \label{lm:nonlip}
% \end{restatable}
% The proof of the first part of the lemma is a direct application of standard concentration inequalities (namely, Hoeffding's inequality to bound $|\sum_{i=1}^n y_i|$, and random matrix theory to bound $\|X\|_{op}$). The proof of the second part of the lemma (presented in the appendix) is via a careful application of the following result due to Adamczak and Wolff, and corresponds to taking $s = d\times k$, and $f(W) := u^\top \overline{z} = u^\top \psi(XW)^\top y$.
% \begin{restatable}[Adamczak-Wolff 2013]{prop}{nonlip}
% \label{prop:nonlip}
% Suppose $W$ is a random vector on $\mathbb R^s$ whose distribution satisfies a log-sobolev inequality with constant $L>0$, and let $f:\mathbb R^s \to \mathbb R$ be a twice-continuously differentiable function with hessian $D^2 f:\mathbb R^s \to \mathbb R^{s \times s}$ which satisfies
% \begin{itemize}
%     \item $\sup_{w \in \mathbb R^s} \|D^2 f(w)\|_{op} \le A_{op}$
%     \item $\sup_{w \in \mathbb R^s} \|D^2 f(w)\|_{HS} \le A_{HS}$
% \end{itemize}
% for some $A_{op}, A_{HS} \ge 0$. Then, for any $t \ge 0$ it holds that
% \begin{eqnarray}
% \mathbb P(|f(w) - \mathbb E[f(w)]| \ge t) \le 2 \exp(-c\frac{t^2}{L^2 \|\mathbb E[\nabla_{\sphere} f(w)]\|^2 + L^4A_{HS}^2} \land \frac{t}{L^2A_{op}}),
% \end{eqnarray}
% where $c>0$ is an absolute constant.
% \end{restatable}
% This result is a generalization of the classical Hanson-Wright inequality for quadratic forms in Gaussian random vectors, to general non-polynomial non-Lipschitz differentiable functions $f:\mathbb R^s \to \mathbb R$ of random vectors satisfying log-sobolev inequalities.
% \paragraph{Emergence of the arc-cosine kernel.}
% Using rotational symmetry of uniform distribution $\sigma_{d-1}$ on the unit-sphere $\sphere$, one computes
% \begin{eqnarray}
% \begin{split}
% \mathbb E_{x \sim \sigma_{d-1}}[v^\top\psi(Wx)] &= \sum_{j=1}^k \mathbb E_x[v_j\psi(u^\top_jx)] = \sum_{j=1}^kv_j\mathbb E_x[\psi(w_j^\top x)]\\
% &=\frac{1}{\sqrt{2\pi d}}\sum_{j=1}^k v_j\|w_j\|
% \end{split}
% \end{eqnarray}
%Thus, $\mathbb E_x[v^\top\psi(Wx)] \le \dfrac{1}{2\pi d}\|v\|^2\|W\|_F^2$.
% \lorem

\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Spectral lower-bound for Lipschitz constant of memorizers]{thm}{}
\label{thm:main}
Let $\psi$ be a $1$-Lipschitz activation function. Then, w.p $1-e^{-\Omega(\sqrt{n} \lor d )}$, any $f=f_{W,v} \in \mathcal F_{d,k}(\psi)$ which memorizes the generic dataset $\mathcal D_n$ must satisfy
\begin{eqnarray}
\Lip_{\sphere}(f) \ge \|\nabla_{\sphere} f\|_{L^2(\sigma_{d-1})} \gtrsim \condnumb_\psi^{-1}(W) \cdot  \frac{\sqrt{n} \lor d}{\sqrt{k}},
\end{eqnarray}
where $\mbox{cond}_\psi^{-1}(W)$ is the spectral ratio defined in \eqref{eq:cond}.
\end{restatable}
\end{mdframed}
The above theorem proves Conjecture \ref{conj:bubeck} \emph{in all regimes where one can show that the condition number $\condnumb_\psi^{-1}(W)$ is lower-bounded}. For example, in the case of ReLU activation, the kernel matrix corresponds to a modified version of the popular arc-cosine kernel, evaluated on the set $\{w_1,\ldots,w_k\}$. This simplifies the above lower-bound (Corollary \ref{cor:cormain}). 
% (i.e $\condnumb_\psi^{-1}(W) \ge c_0$ for some absolute constant $c_0>0$)}.
In the subsequent subsections, we explore some of these regimes.


The proof of Theorem \ref{thm:main} will make use of Theorem \ref{thm:cov} and the following theorem which is of independent importance.

% The following result is one of our main contributions.


\begin{proof}[Proof of Theorem \eqref{thm:main}]
The result then follows by combining \eqref{eq:vnorm}, \eqref{eq:varbound}, and the fact that $\|W\|_{op}^{-1} = \sqrt{\lambda_{\max}(WW^\top )}$ by definition. 
\end{proof}

\subsection{The case of two-layer NNs with no activation: condition number in the usual sense}
Observe that linear models correspond to taking $\psi = \psi_\text{id}$, the identity activation function defined by $\psi_{\text{id}}(t) = t$ for all $t \in \mathbb R$. From \eqref{eq:condlinalg}, we know that
$\condnumb_\psi^{-1}(W) = \dfrac{1}{\condnumb(W)}$,
where $\condnumb(W) := \|W\|_{op}\|W^\dagger\|_{op}$ is the \emph{condition number} of $W$, in the usual sense. Thus, in this case, the lower-bound in Theorem \ref{thm:main} then reduces to
\begin{eqnarray}
\Lip_{\sphere}(f) \ge \|\nabla_{\sphere} f\|_{L^2(\sigma_{d-1})} = \Omega\left(\frac{1}{\condnumb(W)}\cdot \frac{\sqrt n \lor d}{\sqrt k}\right)\text{ w.p }1-e^{-\Omega(\sqrt{n} \lor d)}.
\end{eqnarray}
In particular, if $k=1$, then $\condnumb(W)=1$ and so $\Lip_{\sphere}(f) \ge \|\nabla_{\sphere} f\|_{L^2(\sigma_{d-1})} =\Omega(\sqrt{n} \lor d)$, which is precisely what was proved in Theorem \ref{thm:linthm}.

==> lambdamaxZZ.tex <==
\subsection{Proof of Lemma \ref{lm:lambdamaxZZ}: Bounding the largest eigenvalue of random features gram matrix}
Recall that the setting is that: $W \in \mathbb R^{k \times d}$, $X \in \mathbb R^{n \times k}$, and $Z \in \mathbb R^{n \times k}$ are independent random matrices such that
\begin{itemize}
    \item $W$ (resp. $X$) has independent rows sampled from $\tau_d$, uniform distribution on unit-sphere $\sphere$.
    \item The entries of $Z$ are given for all $(a,j) \in [n] \times [k]$ by $z_{aj} := \sigma(x_a^\top w_j)$ where $\sigma:\mathbb R \to \mathbb R$ is the activation function, which is assumed to continuous and positive-homogeneous of order $1$. Thanks to Lemma 2.2.2 of \cite{Erez2016}, this constraint on $\sigma$ implies the existence of a continuous function $\phi:[-1,1] \to \mathbb R$, which is independent of $n$, $d$, and $k$, such that
    $$
    \mathbb E_{w_j}[z_{aj}z_{bj}] = \frac{1}{d}\phi(x_a^\top x_b).
    $$
\end{itemize}
\lambdamaxZZ*
\begin{proof}
The proof is split into several parts

\emph{(1) Uniform upper-bound for spectral norm of the individual $G_j$'s.}
Standard RMT ~\cite{rmt} tells us that except on an event $\mathcal E$ which occurs w.p $1-e^{-\Omega(1)}$ or less, one has
\begin{eqnarray}
\|X\|_{op} = \mathcal O(1)\text{ w.p }1-e^{-\Omega(d)}.
\end{eqnarray}
Now, $\|\overline{G}_j\|_{op} \le \|G_j\|_{op} + \|\mathbb E_{w_j}[G_j]\|_{op}$, and conditioned on the compliment $\mathcal E'$ of the event $\mathcal E$, one can bound
\begin{eqnarray}
\begin{split}
\|G_j\|_{op}  = \|\sigma(Xw_j)\|^2 &\le \sum_{a=1}^n (x_a^\top w_j)^2 = \|Xw_j\|^2 \le \|X\|_{op}^2 = \mathcal O(1).
\end{split}
\end{eqnarray}
On the other hand, $\|\mathbb E_{w_j}[G_j]\|_{op} = (1/d)\|\phi(XX^\top)\|_{op} = \mathcal O(n/d)=\mathcal O(1)$. Combining with the previous inequality gives $\|G_j\|_{op} = \mathcal O(1)$.

\emph{(2) Upper-bound for pseudo-variance.}
For simplicity, let $\phi_{ab} := \phi(x_a^\top x_b)$, for all $a,b \in [n]$. The $(a,b)$ entry of the $n \times n$ matrix $\mathbb E_{w_j}[\overline{G_j}^2]$ writes
\begin{eqnarray}
\begin{split}
\mathbb E_{w_j}[(\overline{G_j}^2)_{a,b}] &= \sum_{c=1}^n \mathbb E_{w_j}[(\sigma(x_a^\top w_j)\sigma(x_c^\top w_j)-\frac{\phi_{ac}}{d})(\sigma(x_b^\top w_j)\sigma(x_c^\top w_j)-\frac{\phi_{bc}}{d})]\\
&= \sum_{c=1}^n \mathbb E_{w_j}[z_{aj}z_{bj} z_{cj}^2-z_{aj}z_{cj}\frac{\phi_{bc}}{d}-z_{bj}z_{cj}\frac{\phi_{ac}}{d}+\frac{\phi_{ac}\phi_{bc}}{d^2}]\\
&= \sum_{c=1}^n \mathbb E_{w_j}[z_{aj}z_{bj}z_{cj}^2] - \frac{\phi_{ac}\phi_{bc}}{d^2} = \sum_{c=1}^n \mathbb E_{w_j}[z_{aj}z_{bj}z_{cj}^2] - \mathcal O(\frac{n}{d^2}).
\end{split}
\end{eqnarray}
Thus, $|\mathbb E_{w_j}[(\overline{G_j}^2)_{a,b}]| \le \mathcal O(1/d) + \sum_{c=1}^ n\mathbb E_{w_j}[|z_{aj}z_{bj}|z_{cj}^2] \le \mathcal O(1/d) + \mathbb E_{w_j}[|z_{aj}z_{bj}|\sum_{c=1}^n z_{cj}^2]$. By Cauchy-Schwarz inequality, we may bound
$$
(\mathbb E_{w_j}[|z_{aj}z_{bj}|\sum_{c=1}^n z_{cj}^2])^2 \le \mathbb E_{w_j}[z_{aj}^2 z_{bj}^2]\mathbb E_{w_j}[(\sum_{c=1}^n z_{cj}^2)^2].
$$

We bound each factor on the rightmost side like so:
\begin{itemize}
\item[--] $\mathbb E_{w_j}[(\sum_{c=1}^n z_{cj}^2)^2] \le \mathbb E_{w_j}[(\sum_{c=1}^n (x_c^\top w_j)^2)^2] = \mathbb E_{w_j}\|Xw_j\|^4 \le \|X\|^4_{op} = \mathcal O(1)$ on the event $\mathcal E'$, and
\item[--] $\mathbb E_{w_j}[z_{aj}^2z_{bj}^2] \le \|\phi\|_\infty ^2 \mathbb E_{w_j}[(x_a^\top w_j)^2(x_b^\top w_j)^2] = \|\phi\|_\infty^2\dfrac{(x_a^\top x_b)^2}{d(d+2)} \le \mathcal O(\dfrac{1}{d^2})$.
\end{itemize}
Combining with (3) gives $\sup_{a,b \in [n]}|\mathbb E_{w_j}[(\overline{G_j}^2)_{a,b}]| \le \mathcal O(1/d)$ on the event $\mathcal E'$, and so 
$$
v(ZZ^\top):= \sum_{j=1}^k \|\mathbb E_{w_j}[(\overline{G_j}^2)\|_{op} \le k \sup_{j \in [k]} \|\mathbb E_{w_j}[(\overline{G_j}^2)_{a,b}]|\|_{op} \le k \cdot \mathcal O(\frac{n}{d}) = \mathcal O(k)
$$
on the same event, where the third step is thanks to Lemma \ref{lm:eigenpert}.

\emph{(3) Matrix Bernstein inequality.}
By the matrix Bernstein inequality (see Tropp 2015), we obtain that: conditioned on $\mathcal E'$ it holds w.p $1-\delta$ for $\delta = d^{-c}$ (with appropriate $c = \Omega(1)$) that
$$
\|\frac{1}{k}ZZ^\top - \mathbb E_{w_1}[G_1]\|_{op} = \|\frac{1}{k}ZZ^\top - \frac{1}{d}\phi(XX^\top)\|_{op} \le \sqrt{\frac{1}{k}v(ZZ^\top)\log d} + \mathcal O(\frac{\log d}{k})=\mathcal O(\sqrt{\frac{\log d}{k}}),
$$
which proves the first part of the lemma upon recalling that the "bad" event $\mathcal E$ occurs with probability at most $d^{-\Omega(1)}$.

For the second part of the lemma follows from the first: we compute
$$
\|\mathbb E_{w_1}[G_1]\|_{op} = \dfrac{1}{d}\|\phi(XX^\top)\|_{op} \le
\begin{cases}
\mathcal O(1/d),&\mbox{ if }\phi\text{ is "nice"},\\
\mathcal O(n/d)=\mathcal O(1),&\mbox{ else,}
\end{cases}
$$
where the second step is thanks to to ~\cite[Proposition A.2]{justinterpolate}.
\end{proof}

==> ntk.tex <==
\section{Infinite-width RF and NTK regimes}
\input{ntk_intro.tex}


\subsection{Proof of Theorem \ref{thm:infiniteNTKinformal}}
% The spectrum of the RF/NTK matrix $K_{\rf/\ntk}^\infty(X,X)$ will creep up in many computations related to (non)robustness. In the case where $K^\infty_{\rf/\ntk}$ is a dot-product kernel, the following theorem gives asymptotic estimates for the eigenvalues three different interesting sub-regimes.
% \begin{restatable}{cond}{}
% The kernel function $K_{\rf/\ntk}^\infty$ induced by the activation function $\sigma$ is a dot-product type (in the sense of Definition \ref{df:dotprodtype}) and the associated scalar function $\phi^\infty_{\rf/\ntk}:[-1,1] \to \mathbb R$ is continuous on $[-1,1]$,
% twice continuously-differentiable in a neighborhood of \; $0$, with Maclaurin expansion $\phi^\infty_{\rf/\ntk}(\rho)=a_0+a_1\rho + a_2\rho^2 + \mathcal O(\rho^3)$.% Moreover, $\phi^\infty_{\rf/\ntk}$ is positively-curved in the sense of Definition \ref{df:curved}.
% \label{cond:infinitentkcurved}
% \end{restatable}
% \begin{restatable}{rmk}{}
% The above condition is satisfied by a wide range of activation functions, including power $t^p$; power ReLU $\max(t,0)^p$; absolute-value power $|t|^p$; $\mathrm{sign}(t)$; $\tanh(t)$; $\cos(t)$; $\sin(t)$; $\mathrm{erf}(t)$; etc.
% \end{restatable}

\begin{table}[h!]
  \begin{center}
       {\tabulinesep=1.2mm
    \begin{tabu}{|c|c|c|}
    \hline
       Condition & Leading eigenvalue $\lambda_1$ & Other eigenvalues $\lambda_{i\ge 2}$ \\
      \hline
        $a_0=0$, $\alpha>0$ & $\Theta(1)$ & $\Theta(1)$\\
      \hline
        $a_0>0$, $\alpha=0$ & $\Theta(n)$ & $0$\\
      \hline
        $a_0>0$, $\alpha>0$ & $\Theta(n)$ & $\Theta(1)$\\
      \hline
    \end{tabu}
    }
  \end{center}
    \caption{Estimates of the eigenvalues of NTK matrix $K_{\rf/\ntk}^\infty(X,X)$, for dot-product kernels $K_{\rf/\ntk}^\infty(x,x') = \phi(x^\top x)$, where $\phi$ is continuous on $[-1,1]$ and twice-continuously differentiable around $0$ and $a_0 := \phi(0)$, and $\alpha:=\phi(1) - \phi(0) - \phi'(0)$.}
\label{tab:eigH}
\end{table}
% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=.8\linewidth]{Hspec.png}
%     \caption{Graphical illustration of Theorem \ref{thm:eigH}.}
%     \label{fig:Hspec}
% \end{figure}
Presumably, Theorem \ref{thm:eigH} has many useful applications. Let mention one which will be particularly useful for establishing the main result of this section.

\begin{table}[h!]
  \begin{center}
       {\tabulinesep=1.2mm
    \begin{tabu}{|c|c|c|c|}
    \hline
       Activation function $\sigma$ & $\phi^\infty_{\rf/\ntk}(t)$ & Maclaurin expansion & $(\phi^\infty_{\rf/\ntk})'(0)$ \\
      \hline
        ReLU & $\dfrac{t\arccos(-t)}{2\pi}+\mathcal O(\dfrac{1}{d})$ &
        $\dfrac{1}{4}t+\dfrac{1}{2\pi}t^2+\mathcal O(t^3,\dfrac{1}{d})$ & $\dfrac{1}{4}$\\
      \hline
        Absolute value & $\dfrac{2t\arcsin(t)}{\pi}+\mathcal O(\dfrac{1}{d})$ & $\dfrac{2}{\pi}t^2+\mathcal O(t^3,\dfrac{1}{d})$ & $0$ \\
      \hline
        Error function (erf) & $\dfrac{4t}{\pi\sqrt{9-4t^2}}+\mathcal O(\dfrac{1}{d})$ & $\dfrac{4}{3\pi}t+\mathcal O(t^3,\dfrac{1}{d})$ & $\infty$ \\
\hline
    \end{tabu}
    }
  \end{center}
    \caption{Infinite-width RF/NTK kernel function induced by a couple of different activation functions. For the absolute-value activation, we have
    $a_1 = (\phi^\infty_{\rf/\ntk})'(0)$ and so Theorem \ref{thm:infiniteNTKinformal} is inconclusive. For the other activation functions, we have $a_1 \ne 0$, and so the theorem predicts that $\mathfrak{S}(\widehat{f}_{\rf/\ntk}) = \Omega(\sqrt{n})$ w.p $1-d^{-\Omega(1)}$.}
\label{tab:maclaurinkernel}
\end{table}

\subsection{Proof of Lemma \ref{lm:Hy}}
\Hy*
\begin{proof}
For simplicity of notation, set $K:=K^\infty_{\rf/\ntk}(X,X)$. Now, $\|K^{-1} y\|^2 = y^\top K^{-2} y$ a quadratic form in the random vector $y=(y_1,\ldots,y_n)$, with isotropic log-concave distribution. Since $y$ and $X$ are independent and $K$ only depends on $X$, we can use the celebrated Hanson-Wright inequality to obtain that for every $t \ge 0$,
\begin{eqnarray}
\begin{split}
\mathbb P(\left|\|y^\top K^{-2} y - \mathbb E[y^\top K^{-2} y \mid X]\right| < t \mid X) \ge 1-2\exp(-\frac{t^2}{A^2\|K^{-1}\|^2_F} \land \frac{t}{A\|K^{-1}\|_{op}}),
\label{eq:hw}
\end{split}
\end{eqnarray}
where $A>0$ is an absolute constant.

We now simplify the different items appearing in the above display. Let $\lambda_1 \ge \lambda_2 \ge \ldots \ge \lambda_n$ be the eigenvalues of NTK matrix $K$.
Using the fact that $a_0>0$ and $\alpha \ge 0$, we may invoke Theorem \ref{thm:eigH} to deduce that for large $d$ and except on an event $\mathcal E$ which occurs with probability $1-d^{-1+o(1)}$, it holds that $\lambda_n^{-1} \ge \ldots \ge \lambda_2^{-1} = \Theta(1)$ and $\lambda_1^{-1} = \Theta(1/n)$. Conditioned on the event $\mathcal E$, the following estimates are valid.

\emph{-- Controlling the mean.} By the previous paragraph, we know that conditioned on the event $\mathcal E$, $\lambda_n^{-1} = \Theta(1/n)$ and $\lambda_i^{-1} \in [c,C]$ for all $i \in [n]$, where $c,C>0$ are absolute constants. Thus
\begin{eqnarray*}
\begin{split}
\mathbb E[y^\top K^{-2}y \mid \mathcal E] &= \trace(K^{-2}\cov(y)) = \trace(K^{-2})= \sum_{i=1}^n\lambda_i^{-2} \in [c^2n,C^2n].
\end{split}
\end{eqnarray*}
% $$
% \|K^{-1}y\|^2 = \trace(K^{-1}yy^\top K^{-1}) \overset{p}{\longrightarrow} \trace(K^{-2}) = \sum_{i=1}^n \lambda_i^{-2} = \Theta(n),
% % \|K^{-1}y\|_2 \ge \|y\|_2 \cdot \lambda_{\min}(K^{-1}) = \sqrt{n}/\lambda_{1}(K) = \Omega(\sqrt{n}) 
% $$
% which concludes the proof.

\emph{-- Controlling $\|K^{-2}\|_F^2$.} By basic linear algebra, $\|K^{-2}\|_F^2 = \trace(K^{-4}) = \Theta(n)$.

\emph{-- Controlling $\|K^{-2}\|_{op}$.} Finally, we deduce from the previous computation that
$$
\|K^{-2}\|_{op} \le \|K^{-2}\|_F = \Theta(\sqrt{n}),
$$
for some absolute constant $C>0$.
Combining the above with \eqref{eq:hw} we get
$$
\mathbb P(\|K^{-1}y\|^2 - Cn > -t \mid \mathcal E) \ge 1-\exp(-\Omega(\frac{t^2}{n} \land \frac{t}{\sqrt{n}})).
$$
Upon taking $t = (1/2)\mathbb E[y^\top K^{-2} y \mid \mathcal E] \in [(1/2)c^2n,(1/2)C^4n]$, we obtain
\begin{eqnarray*}
\begin{split}
\mathbb P(\frac{c^2n}{2} \le y^\top K^{-2} y \le \frac{3C^2n}{2}) &\ge \mathbb P(-t \le y^\top K^{-2} y - \mathbb E[y^\top K^{-2} y \mid \mathcal E] \le t)\\
&\ge \mathbb P(\mathcal E)\mathbb P(-t \le y^\top K^{-2} y - \mathbb E[y^\top K^{-2} y \mid \mathcal E] \,\Big|\, \mathcal E)\\
% &\ge \mathbb P(|y^\top K^{-2}y - \mathbb E[y^\top K^{-2} y]| < t) = \mathbb P(|y^\top K^{-2}y - \mathbb E[y^\top K^{-2}y]| < n)\\
% & \ge \mathbb P(\mathcal E)\mathbb P(|y^\top K^{-2}-\mathbb E[y^\top K^{-2}y \mid \mathcal E] < n)\\
&\ge \mathbb P(\mathcal E)(1-e^{-\Omega(\frac{(Cn/2)^2}{\Theta(n)} \land \frac{Cn/2}{\Theta(\sqrt{n})})}),\text{ by }\eqref{eq:hw}\\
&= \mathbb P(\mathcal E)(1 - e^{-\Theta(\sqrt{n})})\\
&= (1-d^{-1+o(1)})(1 - e^{-\Theta(\sqrt{n})}),\text{ by construction of }\mathcal E\\
&=1-d^{-1+o(1)},\text{ since }n = \Theta(d).
\end{split}
\end{eqnarray*}
We deduce that $\|K^{-1}y\| = (y^\top K^{-2} y)^{1/2} = \Theta(\sqrt{n})$ w.p $1-d^{-1+o(1)}$ as claimed.

% Using Lemma 4 of Bartlett 20XY, it can be shown that there exist absolute constants $c,C>0$ such that if $z \sim \mathcal N(0,I_n)$, then
% \begin{eqnarray}
% \label{eq:bartlett}
% c \cdot \mathbb E\|K_{\rf/\ntk}^\infty(X,X)^{-1} y\| \le \mathbb E\|K_{\rf/\ntk}^\infty(X,X)^{-1} z\| \le C\log n\cdot\mathbb E\|K_{\rf/\ntk}^\infty(X,X)^{-1} y\|.
% \end{eqnarray}
% Let $\lambda_1 \ge \lambda_2 \ge \ldots \ge \lambda_n$ be the eigenvalues of $K_{\rf/\ntk}^\infty(X,X)$.
% Using the fact that $a_0>0$ and $\alpha \ge 0$, we may invoke Theorem \ref{thm:eigH} to deduce that $\lambda_n^{-1} \ge \ldots \ge \lambda_2^{-1} = \Theta(1)$ in the limit when $n \to \infty$ such that $d/n \in (0,1)$. Thus, by the invariance of the distribution of $z$, we have
% $$
% \mathbb E\|K_{\rf/\ntk}^\infty(X,X)^{-1}z\| = \mathbb E[\|(\lambda_1^{-1} z_1,\ldots,\lambda_n^{-1} z_n)\|\ge \mathbb E\sqrt{\sum_{i=1}^{n-1} \lambda_i^{-2} z_i^2} \ge \lambda_2^{-1} \mathbb E\sqrt{\sum_{i=2}^{n} z_i^2} = \Omega(\sqrt{n}).
% $$
% Combining with \eqref{eq:bartlett} then completes the proof.
\end{proof}

% We are now ready to proof Theorem \ref{thm:nonrobfiniteNTKinformal}. Let us first recall the statement of the theorem.
% \infiniteNTKinformal*

% \begin{proof}
% % [Proof of Theorem \ref{thm:nonrobntk}]% [Proof of Theorem \ref{thm:nonrobntk}]
% %  {\bfseries -- Step 1: Lower-bounding $\|K_{\rf/\ntk}^\infty(X,X)^{-1} y\|$.} Observe that
% % $n = \|y\|^2 = y^\top y = y^\top HK_{\rf/\ntk}^\infty(X,X)^{-1}y$, and so
% % \begin{eqnarray}
% % \label{eq:Hy}
% % \|K_{\rf/\ntk}^\infty(X,X)^{-1} y\| \ge \frac{n}{\|Hy\|} \ge \frac{n}{\|H\|_{op}\|y\|} = \frac{\sqrt{n}}{\|H\|_{op}}.
% % \end{eqnarray}
% % By Hanson-Wright inequality, there exists an absolute constant $c>0$ such that 
% % $$
% % \mathbb P(\|Hy\|^2 - \mathbb E[\|Hy\|^2] \le t) \ge 1- \exp(-\frac{t^2}{\|K_{\rf/\ntk}^\infty(X,X)^2\|^2_{F}} \land \frac{t}{\|K_{\rf/\ntk}^\infty(X,X)^2\|_{op}}).
% % $$
% % Now, $\mathbb E[\|Hy\|^2] = \trace(\cov(y) K_{\rf/\ntk}^\infty(X,X)^2)=\trace(K_{\rf/\ntk}^\infty(X,X)^2) = \|H\|_F^2$. Noting that $\|K_{\rf/\ntk}^\infty(X,X)^2\|_{op} = \|H\|_{op}^2$, $\|H\|_{op} \le \|H\|_F$, $\|K_{\rf/\ntk}^\infty(X,X)^2\|_F^2 \le \|H\|_{op}^2\|H\|_F^2$,  and taking $t=\Omega(n\|H\|_{op}\|H\|_F)$, we obtain that $\|Hy\| = \mathcal O(\sqrt{n\|H\|_{op}\|H\|_F}) = \mathcal O(\sqrt{n}\|H\|_{op})$ w.p $1-e^{-\Omega(n)}$.
% % Combining with \eqref{eq:Hy} then gives $\|K_{\rf/\ntk}^\infty(X,X)^{-1}y\| = \Omega(\sqrt{n}/\|H\|_{op})$ w.p $1-e^{-\Omega(n)}$.
% Invoking \eqref{eq:varbound} of Theorem \ref{thm:cov} with $a=K^\infty_{\rf/\ntk}(X,X)^{-1}y$, and $\Phi=\Phi^\infty_{\rf/\ntk}$ gives
% $$
% \mathfrak{S}(\widehat{f}^\infty_{\rf/\ntk}) \ge \|K^\infty_{\rf/\ntk}(X,X)^{-1}y\|\sqrt{\lambda_{\min}(C_{\Phi^\infty_{\rf/\ntk}})}.
% $$
% where the $n \times n$ random psd matrix $C_{\Phi_{\rf/\ntk}^\infty}=C_{\Phi_{\rf/\ntk}^\infty}(X,X)$ is covariance matrix of the random vector $\Phi_{\rf/\ntk}^\infty(x)$ for $x \sim \tau_d$. Thanks to Lemma \ref{lm:Hy} we now that the first factor above is $\Theta(\sqrt{n})$ w.p $1-d^{-1+o(1)}$ and thanks to Corollary \ref{cor:randV} with $m=n$, $V=X \in \mathbb R^{n \times d}$, and $\varphi=\phi^\infty_{\rf/\ntk}$, we know that the second factor is $\Omega(1)$ w.p $1-e^{-\Omega(d)}$.  Putting these together gives the result immediately.
% \end{proof}


% % $\dfrac{n}{2\|K_{\rf/\ntk}^\infty(X,X)^{-1} y\|} \le \underset{u \in \mathbb S_{n-1}}{\sup}\;z_i(u)$, the supremum of the empirical process $(z_i(u))_{i \in [n],\; u\in \mathbb S_{n-1}}$ defined by $z_i(u) := y_iK_{\rf/\ntk}^\infty(X,X)^\top_i u$, where $h_i$ is the $i$th row of the NTK matrix $K_{\rf/\ntk}^\infty(X,X)$. We shall now upper-bound $Z$ via Bousquet's inequality ~\cite{bousquet2002}. For any $i \in [n]$ and  $u \in \mathbb S_{n-1}$, one computes
% % \begin{itemize}
% %     \item \emph{Wimpy variance.} $\sum_{i=1}^n \mathbb E[z_i(u)^2] = \sum_{i=1}^n (h_i^\top u)^2 = \|Hu\|^2 \le \|H\|_{op}^2$, for all $u \in \mathbb S_{n-1}$.
% %     \item \emph{Mean.} Using standard \emph{Rademacher complexity} arguments, one compute
% %     $$
% %     \mathbb E[Z] = \mathbb E_y \underset{u \in \mathbb S_{n-1}}{\sup}\;\sum_{i=1}^n y_i h_i^\top u \le \sqrt{\sum_{i=1}^n \|h_i\|^2} = \|H\|_{F}.
% %     $$
% % \end{itemize}
% % Define $\nu = 2\mathbb E[Z] + \underset{u \in \mathbb S_{n-1}}{\sup}\;\sum_{i=1}^n \mathbb E[z_i(u)^2] \le 2\|H\|_F + \|H\|_{op}^2$

% % \subsection{Other examples}
% % \paragraph{Power activation function}

% % \lorem

% % \lorem

% \section{Finite-width NTK regime (proof of Conjecture \ref{conj:bubeck})}
% \label{sec:finiteNTK}
% We now consider a finite-rank NTK $f(x) = a^\top \Phi_{\rf/\ntk}(x)$, where the feature map $\Phi_{\rf/\ntk}:\sphere \to \mathbb R^{kd}$ is defined by
% \begin{eqnarray}
% \Phi_{\ntk}(x) := \frac{1}{\sqrt{k}}
% (\sigma'(x^\top w_1)x,\ldots,\sigma'(x^\top w_k)x) \in \mathbb R^{kd},
% \end{eqnarray}
% where $W = (w_1,\ldots,w_k) \tau_d^{\otimes k}$ is the random matrix of hidden neuron weights and $a \in \mathbb R^{kd}$ is the vector of learnable parameters.
% The corresponding empirical kernel matrix is the $n \times n$ psd matrix
% $K_{\rf/\ntk}(X,X)$, defined by
% \begin{eqnarray}
% (K_{\ntk}(X,X))_{i,\ell}  = \Phi_\ntk(x_i)^\top \Phi_\ntk(x_\ell) = \frac{1}{k}\sum_{j=1}^k \sigma'(x_i^\top w_j)\sigma'(x_i^\top w_\ell)x_i^\top x_\ell,
% \end{eqnarray}
% i.e $K_\ntk(X,X) := ZZ^\top$, where $Z:=\Phi_\ntk(X) \in \mathbb R^{n \times kd}$.
% This is just a finite-width approximation of the infinite-width NTK matrix defined in \eqref{eq:infinitentk}, with only the first-layer kernel.
% \begin{restatable}[\cite{montanari2020}]{prop}{}
% Define $\eta(\sigma) := \var(\sigma'(z))$, for $z \sim N(0,1)$, and assume $\eta(\sigma) > 0$. In the limit when $n,k,d \to \infty$ in the sense of \eqref{eq:anormfinitentk}, it holds that

% \begin{eqnarray}
% \begin{split}
% \lambda_{\min}(K_\ntk(X,X)) &\ge \eta(\sigma)-o_{\mathbb P}(1). % ,\\
% % \lambda_{\max}(K_\ntk(X,X)) &= \mathcal O_{\mathbb P}(1).
% \end{split}
% \end{eqnarray}
% \label{prop:montanari}
% \end{restatable}
% In particular, one deduces from the above result that $\rank(K_\ntk(X,X)) = n$, and so w.h.p the (finite-rank) NTK model $\widehat{f}_\ntk$ given in \eqref{eq:ntkfinite}
% memorizes the generic dataset $\mathcal D_n$.

% For a ridge penalty parameter $\lambda > 0$, one is let to consider the optimization problem \eqref{eq:finitentkest} with solution $\widehat{a}=(Z^\top Z + \lambda I_{kd})^{-1} Z^\top y$, to get a corresponding fitted NTK model
% \begin{eqnarray}
% \label{eq:ntkfinite}
% \widehat{f}_\ntk(x)=\Phi_\ntk(x)^\top (Z^\top Z + \lambda I_{kd})^{-1} Z^\top y = (Z\Phi_\ntk(x))^\top (K_\ntk(X,X)+\lambda I_n)^{-1}y.
% \end{eqnarray}
% % The methods of \cite{elkaroui2010} etc., cannot work and we need to do something else.

% \subsection{Proof of Theorem \ref{thm:nonrobfiniteNTKinformal}}
% \label{sec:prooffinitentk}
% % \begin{restatable}[Almost-optimal parametrization]{cond}{}
% % $n,d,k \to \infty$ such that the following holds
% % \begin{eqnarray}
% % (\log k)^C = o(d),\; (\log d)^C = o(k),kd \ge n(\log d)^{C_0},
% % \label{eq:almost}
% % \end{eqnarray}
% % for some absolute constant $C_0>0$, and for every $C>0$.
% % \label{cond:almost}
% % \end{restatable}
 

% Playing games similar to what we did in the previous subsection, we have

% \begin{restatable}{lm}{}
% For $x \sim \tau_d$, the covariance matrix of $\Phi_\ntk(x)$ is given by
% $$
% C_{\Phi_{\ntk}} = \frac{1}{k}(\Sigma_{\sigma'}(W,W) \otimes I_d) \in \mathbb R^{kd \times kd},
% $$
% where $\Sigma_{\sigma'}(W,W)$ is the covariance matrix of $\sqrt{d}\sigma'(Wx)$, with entries given for all $j,\ell \in [k]$ by 
% $$
% \Sigma_{\sigma'}(w_j,w_\ell):= \mathbb E_x[\sqrt{d}\sigma'(x^\top w_j)\sqrt{d}\sigma'(x^\top w_\ell)]-\mathbb E_x[\sqrt{d}\sigma'(x^\top w_j)]\mathbb E_x[\sqrt{d}\sigma'(x^\top w_\ell)].
% $$
% \end{restatable}
% \begin{proof}
% Let $x \sim \tau_d$ and $z(x) := (1/\sqrt{k})\sigma'(Wx) := ((1/\sqrt{k})\sigma'(x^\top w_1),\ldots,(1/\sqrt{k})\sigma'(x^\top w_k)) \in \mathbb R^k$, and observe $\Phi_\ntk(x) = z(x) \otimes x \in \mathbb R^{kd}$, the Kronecker product of $z(x)$ and $x$. On the other hand, it is clear that $z(x)$ and $x$ are independent. Thus using a well-known result for the covariance of the Kronecker product of independent random vectors, we obtain
% $$
% C_{\Phi_\ntk} = d\cdot \cov(z(x) \otimes x) = d\cdot \cov(z(x)) \otimes \cov(x) = \frac{d}{k}\Sigma_{\sigma'}(W,W) \otimes \frac{1}{d}I_d=\frac{1}{k}\Sigma_{\sigma'}(W,W) \otimes I_d,
% $$
% as claimed.
% \end{proof}

% We are now ready to attack Theorem \ref{thm:nonrobfiniteNTKinformal}, whose statement we first recall.
% \nonrobfiniteNTKinformal*

% \begin{proof}
% % $\nabla \widehat{f}_\ntk(x) = (z(x) \otimes I_d)a=(z(x)^\top a_1,\ldots,z(x)^\top a_k) \in \mathbb R^d$, where $a = (a_1,\ldots,a_k)$, with $a_j \in \mathbb R^d$ for all $j \in [k]$. Thus $\|\nabla_{\sphere}\widehat{f}_\ntk(x)\|^2 = \|\nabla \widehat{f}_\ntk(x)\|^2 - (\widehat{f}_\ntk(x))^2 \le \|A^\top z(x)\|^2$, and so,
% % $\|\nabla_{\sphere} \widehat{f}_\ntk\|_{L^2(\tau_d)}^2 = \mathbb E_x[\|A^\top z(x)\|^2] \le \|A\|_{op}^2\mathbb E_x \|z(x)\|^2 \le \|A\|_{op}^2 \le \|A\|_F^2$.
% Thanks to Theorem \ref{thm:cov}, one has
% \begin{eqnarray}
% \begin{split}
% \mathfrak{S}(\widehat{f}_{\ntk,\lambda})^2 &\ge d \cdot \|\widehat{a}_\ntk(\lambda)\|^2\lambda_{\min}(C_{\Phi_\ntk}) = \|\widehat{a}_\ntk(\lambda)\|^2\lambda_{\min}(\frac{1}{k}\Sigma_{\sigma'}(W,W)\otimes I_d)\\
% &= \frac{\|\widehat{a}_\ntk(\lambda)\|^2}{k}\lambda_{\min}(\Sigma_{\sigma'}(W,W)) = \Omega(\frac{\|\widehat{a}_\ntk(\lambda)\|^2}{k}) \text{ w.p }1-d^{-\Omega(1)},
% \end{split}
% \label{eq:Fk}
% \end{eqnarray}
% since $\lambda_{\min}(\Sigma_{\sigma'}(W,W)) = \lambda_{\min}(K_{\sigma'}(WW^\top)) = \Omega(1)$ w.p $1-d^{-\Omega(1)}$ thanks to Corollary \ref{cor:Cspecrelu}. %  (applicable here since $k \asymp d$).

% Next, thanks to \eqref{eq:anormfinitentk}, we know that $\|\widehat{a}_\ntk(\lambda)\|^2 = \Omega_{\mathbb P}(n)$ for $\lambda = \mathcal O(1/n)$.
% % Now,  because $n \lesssim n(\log d)^{C_0} \le kd$, the finite-width empirical NTK kernel matrix $K_\ntk(X,X)$ is invertible w.p $1$ and so the regression coefficients are given by $a = \Phi_\ntk(X)^\top K_\ntk(X,X)^{-1}y$. In particular, $\|a\|^2 = y^\top K_\ntk(X,X)^{-1} y$. Since the eigenvalues of $K_\ntk(X,X)$ are almost-surely uniformly bounded thanks to Proposition \ref{prop:montanari}, we deduce that $\|K_\ntk(X,X)^{-1}\|_F = \mathcal O_{\mathbb P}(\sqrt{n})$. Thus, we can apply Hanson-Wright in an analogous way we did in the proof of Lemma \ref{lm:Hy} (except that now "w.p $1-d^{-\Omega(1)}$" must now be replaced with "almost-surely"), to get
% % $\|a\|^2 = \Omega_{\mathbb P}(n)$.
% Combining with \eqref{eq:Fk} then gives the result.
% % \begin{eqnarray}
% % \begin{split}
% % \|A\|_F^2 &= \trace(y^\top K_\ntk(X,X)^{-1}\Phi_\ntk(X)\Phi_\ntk(X)^\top K_\ntk(X,X)^{-1}y)\\
% % &= \trace(y^\top K_\ntk(X,X)^{-1} y) \overset{a.s}{\to} \trace(K_\ntk(X,X)^{-1})\\
% % &= \trace(K_\ntk^{\mathrm{lin}}(X,X)^{-1}) + o_{\mathbb P}(1)= \Omega_{\mathbb P}(n),
% % \end{split}
% % \end{eqnarray}
% % where $K_\ntk^{\mathrm{lin}}(X,X) := \eta(\sigma) I_n + \zeta(\sigma) XX^\top + c(\sigma)R $, with $\eta(\sigma) := (\mathbb E_{z \sim N(0,1)}\sigma'(z))^2$, and we have used the fact that $K_\ntk^{\mathrm{lin}}(X,X)$ and $K_\ntk(X,X)$ asymptotically have the same statistics for their bulk eigenvalues (thanks to Pennington et al. 20XY). Here, $R$ is a rank-1 matrix (and thus does not affect the bulk statistics of the eigenvalues of $K_\ntk^{\mathrm{lin}}(X,X)$.
% \end{proof}

% % \section{Nonlinear random matrix theory}
% % \subsection{Extending a result of Pennington and Worah}
% % Note that if $\sigma(z)$ has finite moments up to order to $z$ w.r.t $z \sim N(0,1)$, then by taking $\alpha := \mathbb E_{z \sim N(0,1)}[\sigma(z)]$ and then renormalizing by the standard deviation of $\sigma(z)$,
% % one can decompose the activation function $\sigma:\mathbb R \to \mathbb R$ as $\sigma(x) = \alpha + \widetilde{\sigma}(x)$, where $\alpha \in \mathbb R$, and $\widetilde{\sigma}:\mathbb R \to \mathbb R$ is a "purely nonlinear" activation function in the sense that
% % \begin{eqnarray}
% % \mathbb E_{z \sim N(0,1)}[\widetilde{\sigma}(z)] = \mathbb E_{z \sim N(0,1)}[z\widetilde{\sigma}(z)] = 0, \;\mathbb E_{z \sim N(0, 1)}[\widetilde{\sigma}(z)^2] = 1.
% % \end{eqnarray}

% % For $W \sim N(0,1)^{k \times d}$, let $Z=Z(X,W)$ and $\widetilde{Z}=\widetilde{Z}(X,W)$ be $n \times k$ random matrices with entries defined defined by $z_{ij} = \sigma(x_i^\top w_j)$ and $\widetilde{z}_{ij} := \widetilde{\sigma}(x_i^\top w_j)$ for all $i \in [n]$ and $j \in [k]$.
% % \begin{restatable}[Corollary 6 of ~\cite{Hastie2019}]{prop}{}
% % If $\widetilde{\sigma}$ satisfies $|\widetilde{\sigma}(x)| \le c_0(1+|x|)^{c_1}$ for some absolute constants $c_0,c_1>0$ and for all $x \in \mathbb R$, then $\mathrm{LSD}(\widetilde{Z}\widetilde{Z}^\top) \to \mu_\gamma^\MP$ weakly, in the limit $n,d,k \to \infty$ according to \eqref{eq:proportionate}.
% % \end{restatable}
% % We will extend this result to capture the LSD of $ZZ^\top$, the full nonlinear feature empirical covariance matrix. Note that $Z = \widetilde{Z}+A$, where $A:=\alpha 1_n 1_k^\top$ is the all-ones matrix of shape $n \times k$, times the scalar $\alpha$. Also note that that $AA^\top=k\alpha^2 1_n1_n^\top$. Thus, we have the decomposition $ZZ^\top  = \widetilde{Z}\widetilde{Z}^\top + A\widetilde{Z}^\top + \widetilde{Z}^\top A + AA^\top$.
% % The next Lemma shows that except for a few isolated large eigenvalues (due to the rank-one perturbation $A$), the bulk of the empirical eigenvalue distribution of $\widetilde{Z}\widetilde{Z}^\top$ matches that of $ZZ^\top$. This approximation will be sufficient to get a good approximation involving the the empirical eigenvalues of $\widetilde{Z}\widetilde{Z}^\top$, which is itself an almost-sure limit for the squared $L_2$-norm of the output weights vector of $f^{\mathrm{RF}}$, namely $\trace((\widetilde{Z}\widetilde{Z}^\top)^{-1})$.
% % \begin{restatable}{lm}{}
% % There exists an absolute constant $c>0$ such that in the limit $n,d,k \to \infty$, it holds almost surely that
% % $\lambda_i(ZZ^\top) \to \lambda_i(\widetilde{Z}\widetilde{Z}^\top) + kn\alpha^2 1_{i=1}$ for every $i \in [n]$ with $n \ge c$.
% % \label{lm:rankone}
% % \end{restatable}

% % \mytodo{Integrate Theorem 2.1 of \url{https://arxiv.org/pdf/0910.2120.pdf}}

% % \begin{figure}[!htp]
% %     \centering
% %     \includegraphics[width=.8\linewidth]{golub.png}
% %     \caption{Experimental illustration of Lemma \ref{lm:rankone}, with $Z \sim N(0,1)^{n \times k}$, with $n=800$, $k=1000$, and $\alpha=1/\sqrt{nk}$.}
% %     \label{fig:my_label}
% % \end{figure}
% % \begin{proof}[Sketch of proof]

% % We only sketch the key ideas.

% % {\bfseries -- Fact 1.} $\mbox{LSD}(ZZ^\top) = \mbox{LSD}(\widetilde{Z}\widetilde{Z}^\top + A\widetilde{Z}^\top + \widetilde{Z}^\top A + AA^\top) \to \mbox{LSD}(\widetilde{Z}\widetilde{Z}^\top + AA^\top)$ weakly.

% % % The above fact (it seems) was implied by Ofer's comment. I've observed this empirically, but I'm not quite sure why it should be true. Maybe this is a consequence of some classical / well-known lemma from *free probability theory* ?

% % Also, invoking result due to G. Golub and V. Loan, we deduce that

% % {\bfseries -- Fact 2.} There exist $q_1,\ldots,q_n \ge 0$ with $\sum_{i=1}^n q_i = 1$, such that $$
% % % \lambda_i(\widetilde{Z}\widetilde{Z}^\top+AA^\top) = 
% % \lambda_i(\widetilde{Z}\widetilde{Z}^\top + k\alpha^2 1_n1_n^\top) = \lambda_i(\widetilde{Z}\widetilde{Z}^\top) + q_i nk\alpha^2\;\forall i \in [n].
% % $$
% % Moreover, one has the explicit formula $q_i = \dfrac{(1_n^\top a_i)(1_n^\top b_i)}{n a_i^\top b_i}$ (provided $a_i^\top b_i \ne 0$), where $a_1,\ldots,a_n$ are the eigenvectors of $\widetilde{Z}\widetilde{Z}^\top$ and $b_1,\ldots,b_n$ are the eigenvector of $b_i$. Intuitively, one whould expect $a_i$ to be pretty much orthogonal to $b_i$ for $i \ne 1$. As a consequnce, one would expect $q \to \delta_{i=1} \in \ell^2$ almost-surely.

% % Putting all the bits together (and of course making some of the above arguments rigorous) completes the proof.
% % \end{proof}

% % \begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
% % \begin{restatable}{thm}{}
% % Suppose the activation function $\sigma$ has unit variance and satisfies w.r.t $z \sim N(0,1)$. Also suppose $|\sigma(x)| \le c_0(1+|x|)^{c_1}$ for absolute constants $c_0,c_1 \ge 0$, and for all $x \in \mathbb R^d$. Then there exists $t \in (0,1]$ such that $\mathrm{LCD}(ZZ^\top) \to t\mu_\gamma^\MP+(1-t) \delta_{nk\eta^2}$ weakly.
% % \label{thm:lsd}
% % \end{restatable}
% % \end{mdframed}
% % \begin{proof}
% % \lorem
% % \end{proof}
% % \begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
% % \begin{restatable}{cor}{}
% % Under the conditions of Theorem \ref{thm:lsd}, in the limit Let $n,d,k \to \infty$ according to \eqref{eq:proportionate}, we have
% % $$
% % n^{-1}\trace((ZZ^\top)^{-1}) \to \frac{1}{1-\gamma}\text{ almost-surely}.
% % $$
% % \end{restatable}
% % \end{mdframed}

% % \begin{proof}
% % Thanks to Lemma \ref{lm:rankone}, we have
% % $$
% % n^{-1}\trace((ZZ^\top)^{-1}) = \dfrac{1}{n}\sum_{i=1}^n \dfrac{1}{\lambda_i(ZZ^\top)}=\dfrac{1}{n}\sum_{i=1}^n \dfrac{1}{\lambda_i(ZZ^\top)} + \mathcal O(\dfrac{1}{nk}) \overset{a.s}{\to} \int \frac{1}{t}\dif \mu_\gamma^{\MP}(t),
% % $$
% % and the proof is completed by noting that $\int \dfrac{1}{t}\dif \mu_\gamma^\MP(t) = \dfrac{1}{1-\gamma}$.
% % \end{proof}

==> ntk_intro.tex <==
% \lorem
\label{sec:asympntk}
We place ourselves in an infinite-width NTK where the number of neurons is $k = \infty$, and $n \asymp d$ modulo logarithmic factors in $d$.
% It is known (cite Arora XYZ) that the resulting linear model \eqref{eq:ntkreg} can actually memorize generic data.
Let $\theta = (W,v)$ be a the parameters of a two-layer neural network $f_{W,v} \in \mathcal F_{d,k}(\sigma)$ and and consider a psd kernel $K^\infty_{\rf/\ntk}$ on $\mathcal S_{d-1}$ defined by \cite{jacot18,inductivebietti,montanari2020}
\begin{eqnarray}
K^\infty_{\rf/\ntk}(x,\widetilde{x}) := \mathbb E_{\theta} [\nabla_\theta f(x)^\top \nabla_\theta f(\widetilde{x})] = K_1(x,\widetilde{x})+K_2(x,\widetilde{x}),\text{ for all }x,\widetilde{x} \in \mathcal S_{d-1},
\end{eqnarray}
where $K_2$ and $K_2$ are the second- and first-layer kernels respectively, defined by $K_2(x,\widetilde{x}):= \mathbb E_{w \sim \tau_d}[\sigma'(x^\top w)\sigma'(\widetilde{x}^\top w)]$ and $K_1(x,\widetilde{x}) = \mathbb E_{w \sim \tau_d}[\sigma(x^\top w)\sigma(\widetilde{x}^\top w)]$. Taking $\theta=W$ leads to $K_{\rf/\ntk}^\infty = K_\rf = K_1$, the infinite-width pure RF kernel; taking $\theta=v$ gives $K^\infty_{\rf/\ntk} = K_\ntk = K_2$, the infinite-width pure NTK kernel.
% Note that the expectation is taken over random $W$ with iid entries from $N(0,1/d)$, and random $v$ with iid entries from $N(0,1/k)$.

Now, for any input $x \in \mathcal S_{d-1}$, define the feature vector $\Phi^\infty_{\rf/\ntk}(x) \in \mathbb R^n$ by $$
\Phi^\infty_{\rf/\ntk}(x):=K_{\rf/\ntk}^\infty(x,X):=(K^\infty_{\rf/\ntk}(x,x_1),\ldots,K^\infty_{\rf/\ntk}(x,x_n)).
$$
Finally, define the corresponding NTK as the $n \times n$ matrix $K_{\rf/\ntk}^\infty(X,X)$ defined by
\begin{eqnarray}
\label{eq:infinitentk}
(K^\infty_{\rf/\ntk}(X,X))_{i,\ell} := K^\infty_{\rf/\ntk}(x_i,x_\ell).
\end{eqnarray}

Since $x_1,\ldots,x_n \sim \tau_d$ (i.e uniform iid on the unit-sphere $\sphere$), w.p $1$ no two of them are parallel. Thus, $K_{\rf/\ntk}^\infty(X,X)$ is invertible w.p $1$. Now, consider the so-called "NTK regressor" defined by
\begin{eqnarray}
\widehat{f}^\infty_{\rf/\ntk}(x) := \underbrace{\Phi^\infty_{\rf/\ntk}(x)^\top}_{\text{features}} \underbrace{K^\infty_{\rf/\ntk}(X,X)^{-1}y}_{\text{regression coefficients}}.
\label{eq:ntkreg}
\end{eqnarray}
For simplicity, we only consider the unregularized / ridgeless scenario.
It is known that gradient-flow on squared loss converges to $\widehat{f}_{\rf/\ntk}^\infty$.
It is clear that $\widehat{f}_{\rf/\ntk}^\infty$ memorizes the dataset $\mathcal D_n$ (with zero error!). The goal of this section is to prove that this memorization is far from being robust, or more precisely, that $\mathfrak{S}(\widehat{f}^\infty_{\rf/\ntk})= \Omega(\sqrt{n})$ with overwhelming probability.

Note that this model is an instance of \eqref{eq:featurized} and \eqref{eq:Vmodel} with  $m=n$ (the sample size), $a := K^\infty_{\rf/\ntk}(X,X)^{-1}y \in \mathbb R^n$ and feature mapping $\varphi=\kappa^\infty_{\rf/\ntk}$, $V=X \in \mathbb R^{n \times d}$.

% \subsection{A trivial bound}
% \lorem

==> oldfinite.tex <==


\subsection{A generic law via a new kind of condition number}
% We will now show that with overwhelming probability, a two-layer neural network $f_{W,v} \in \mathcal F_{d,k}(\sigma)$ which memorizes the generic dataset $\mathcal D_n$ must satisfy $\|v\|\|W\|_{op} \ge \Omega(\sqrt{n/k})$.

Define a funciton $\eta:\mathbb R^{k \times d} \times \mathbb R^k \to \mathbb R$ by
\begin{eqnarray}
\begin{split}
    \eta(W,v) &:= \sum_{j=1}^k |v_j|\|w_j\|_2.
\end{split}
\end{eqnarray}
By basic results for $\ell_p$ norms in $\mathbb R^d$, we may relate $\eta_1$ and $\eta_2$ as follows
\begin{eqnarray}
\begin{split}
\sqrt{k}\|v\|\|W\|_{op} &\ge \sqrt{k}\|v\|_2\max_{j \in [k]}\|w_j\|_2 \ge \|v\|_1\max_{j \in [k]}\|w_j\|_2\ge \sum_{j=1}^k |v_j|\|w_j\|_2 =: \eta_2(W,v).
\end{split}
\end{eqnarray}
This proves the following basic lemma which will be useful in a bit.
\begin{restatable}{lm}{}
For all $W \in \mathbb R^{k \times d}$ and $v \in \mathbb R^k$, it holds that $\|v\|\|W\|_{op} \ge \dfrac{\eta(W,v)}{\sqrt{k}}$. 
\end{restatable}

For $R \ge 0$, let $\mathcal B_{d,k}(\sigma,R) := \{f=f_{W,v} \in \mathcal F_{d,k}(\sigma) \mid \eta(W,v) \le R\}$. Give a matrix $W \in \mathbb R^{k \times d}$, let $\mathcal F_W(\sigma) \subseteq \mathcal F_{d,k}(\sigma)$ denote the subclass of all two-layer neural networks with activation function $\sigma$ and hidden weights matrix fixed at $W$.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Law of robustness for two-layer neural network with fixed hidden weights]{thm}{}
For every $\varepsilon \in [0,\varepsilon^\star)$, it holds w.p $1-d^{-\Omega(1)}$ over $\mathcal D_n$ that: every $f \in \mathcal F_W(\sigma)$ with $\widehat{\varepsilon}_n(f) \le \varepsilon$ must verify
\begin{eqnarray}
\mathfrak{S}(f) \ge \Omega(\frac{(\varepsilon^\star-\varepsilon)}{\alpha_\sigma(W)}\sqrt{\frac{n}{k}}),
\end{eqnarray}
where $\alpha_\sigma(W) := \dfrac{\lambda_{\max}(WW^\top)}{\lambda_{\min}(C_\sigma(W))}$ is the "condition number" of $W$ w.r.t $\sigma$.
\label{thm:generalnnbound}
\end{restatable}
\end{mdframed}
Motivation for the name "condition number of $W$ w.r.t $\sigma$" comes from the fact that if $\sigma$ is the identity activation function, then $C_\sigma(W) = \cov_{x \sim \tau_d}(\sqrt{d} Wx) = W\cov_{x \sim \tau_d}(\sqrt{d} x)W^\top = WW^\top$, and so $\alpha_\sigma(W) = \lambda_{\max}(WW^\top)/\lambda_{\min}(WW^\top)$, which is the ordinary condition number (linear algebra) of the matrix $W$.
\begin{proof}[Proof of Theorem \ref{thm:generalnnbound}]
By Theorem 2 of CS229T/STATS231: Statistical Learning Theory, w.p $1-\delta$, it holds that
$$
\varepsilon^\star \le \mathbb P(yf(x) \le 0) \le \widehat{\varepsilon}_n(f)+\mathcal O(\frac{R}{\sqrt{n}})+\sqrt{\frac{\log(2/\delta)}{n}}\,\forall f \in \mathcal B_{d,k}(\sigma,R).
$$
Taking $\delta = d^{-c}$ (for appropriate $c=\Omega(1)$) and rearranging gives that for every $f \in \mathcal B_{d,k}(\sigma,R)$, it holds w.p $1-d^{-\Omega(1)}$ over $\mathcal D_n$ that $\mathcal B_{d,k}(\sigma,R)$ contains no $f$ with $\widehat{\varepsilon}_n(f) \le \varepsilon$ unless
$R \ge \widetilde{\Omega}((\varepsilon^\star-\varepsilon)_+\sqrt{n})$. We deduce that w.p $1-d^{-c}$, every $f=f_{W,v} \in \mathcal F_{d,k}(\sigma)$ with $\widehat{\varepsilon}_n(f) \le \varepsilon$ must verify (recall that $\widetilde{\Omega}(\ldots)$ is notation for lower-bounds hiding constant and log factors in $n$) 
\begin{eqnarray}
\|v\|\|W\|_{op} =: \eta_1(W,v) \ge \frac{\eta_2(W,v)}{\sqrt{k}} \ge \widetilde{\Omega}((\varepsilon^\star-\varepsilon)\sqrt{\frac{n}{k}}).
\end{eqnarray}
The result then follows upon combining this with Theorem \ref{thm:analytic} via \eqref{eq:sandwitch}.
\end{proof}

\subsection{Detailed spectral analysis of $C_\sigma(W)$ for specific activation functions}
\label{subsec:rfspec}
We now specialize Lemma \ref{lm:specC} to the case where the activation function $\sigma$ is the ReLU or the absolute-value.
We have the following important corollary to Lemma \ref{lm:specC}.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Extreme eigenvalues of kernel random matrix in case of ReLU activation function]{cor}{}
% Suppose the rows $w_1,\ldots,w_k$ are drawn iid uniformly from $\sphere$ of the hidden weights matrix $W \in \mathbb R^{k \times d}$, and 
% the activation function $\sigma$ is the ReLU.
For the ReLU activation function $\sigma(t) = \max(t,0)$, we have the following
\begin{itemize}
\item[(A)] Lower-bound on smallest eigenvalues of $C_\relu(W,W)$: for sufficiently large $d \asymp k$, it holds w.p $1-d^{-1+\Omega(1)}$ over the choice of $W$ that
$$
\lambda_{\min}(C_\relu(W,W)) \ge \dfrac{\pi-2}{4\pi}-\mathcal O(\frac{1}{d}) =\Omega(1).
$$
\item[(B)] Upper-bound on largest eigenvalue of $C_\relu(W,W)$:
In the limit $d,k \to \infty$ with $\limsup k/d \in (0,\infty)$, we have
$
\lambda_{\max}(C_\relu(W,W)) = \mathcal O_{\mathbb P}(1).
$
% \begin{eqnarray}
% \|C_\sigma(W) - \frac{1}{4}WW^\top+1)\|_{op} = \mathcal O(d^{-1/2}\log^{0.51} d):
% \end{eqnarray}
% \item[(A)] Estimation of eigenvalues of $C_\sigma(W)$: If $\lambda_{\max} = \lambda_1 \ge \ldots \ge \lambda_k = \lambda_{\min}$ are the eigenvalues of $C_\sigma(W)$ and $\overline{\lambda}_1 \ge \ldots \ge \overline{\lambda}_k $ are the eigenvalues of $WW^\top$, then
% \begin{eqnarray}
% \lambda_j = \frac{1}{4}\overline{\lambda}_j + \frac{2\pi-4}{4\pi} + \mathcal O(d^{-1/2}\log^{0.51} d),\text{ for all }j \in [k].
% \end{eqnarray}
% \item[(B)] Estimation of extreme eigenvalues of $C_\sigma(W)$. It holds that
% $\lambda_{\min} \ge \dfrac{2\pi-4}{4\pi}-o(1)$ and $\lambda_{\max}= \mathcal O(1)$.
\end{itemize}
\label{cor:Cspecrelu}
\end{restatable}
\end{mdframed}
% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{Cspec.png}
%     \caption{Empirical verification of Corollary \ref{cor:Cspecrelu} with $k=100$ and $d=150$.}
%     \label{fig:Cspec}
% \end{figure}
\begin{proof}
Thanks to Table \ref{tab:maclaurin}, the Maclaurin expansion of $\widetilde{\kappa}_\relu$ writes
$
\widetilde{\kappa}_\relu(t) =a_0+a_1t+at^2 + \mathcal O(t^3),
$
where the coefficients $a_0$, $a_1$, and $a$ are given by
\begin{eqnarray*}
\begin{split}
    a_0 = 1/4+\mathcal O(1/d),\, a_1=\widetilde{\kappa}_\relu'(0) = 1/(2\pi) + \mathcal O(1/d),\,a_2 =\mathcal O(1/d).
\end{split}
\end{eqnarray*}
We deduce that the El Karoui curvature coefficients of $\widetilde{\kappa}_\relu$ are $\beta_1 := a_0 = 1/4+\mathcal O(1/d)$, $\beta_2 := a_1 = 1/(2\pi) + \mathcal O(1/d)$, and $\beta_3 := \widetilde{\kappa}_\relu(1) - a_1 - a_2 = 1/(2\pi)-1/4-1/(2\pi) - \mathcal O(1/d)=(\pi-2)/(4\pi)-o(1)$. Thanks to Lemma \ref{lm:specC}, we know that $\|C_\relu(W,W) - C^{\mathrm{lin}}_\relu(W,W)\|_{op} = o(1)$ w.p $1-d^{-1+o(1)}$ where $C_\sigma(W)^{\mathrm{lin}} := \beta_1 1_k1_k^\top + \beta_2 WW^\top + \beta_3 I_k$. The first part of the claim follows from the fact that $C_\sigma(W)^{\mathrm{lin}} \ge \beta_3 I_k$. The second part follows from standard RMT and fact that in the limit $d \to \infty$, the rank-1 perturbation $\beta_2 1_k1_k^\top$ does not change the spectrum of $C^{\mathrm{lin}}_\relu(W,W)$.
\end{proof}

\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Extreme eigenvalues of kernel random matrix in case of absolute-value activation function]{cor}{}
% Suppose the rows $w_1,\ldots,w_k$ are drawn iid uniformly from $\sphere$ of the hidden weights matrix $W \in \mathbb R^{k \times d}$, and 
% the activation function $\sigma$ is the ReLU.
Consider the absolute-value activation function $\sigma(t) = |t|$. For sufficiently large $d \asymp d$, we have the following bound for the extreme eigenvalues of $C_\abs(W,W)$
$$
1-\mathcal O(1/d) \le \lambda_{\min}(C_\abs(W,W)) \le \lambda_{\max}(C_\abs(W,W)) \le 1 + \mathcal O(1/d).
$$
\label{cor:Cspecabs}
\end{restatable}
\end{mdframed}
\begin{proof}
Thanks to Table \ref{tab:maclaurin}, the Maclaurin expansion of $\widetilde{\kappa}_\abs$ writes
$
\widetilde{\kappa}_\abs(t) =a_0+a_1t+at^2 + \mathcal O(t^3),
$
where the coefficients $a_0$, $a_1$, and $a$ are given by
\begin{eqnarray*}
\begin{split}
    a_0 = \mathcal O(1/d),\, a_1 = \mathcal O(1/d),\,a_2 =2/\pi +\mathcal O(1/d).
\end{split}
\end{eqnarray*}
We deduce that the El Karoui curvature coefficients of $\widetilde{\kappa}_\abs$ are $\beta_1 := a_0= \mathcal O(1/d)$, $\beta_2 := a_1 = \mathcal O(1/d)$, and $\beta_3 := \widetilde{\kappa}_\abs(1) - a_1 - a_2 = 2/\pi+\mathcal O(1/d)$. Thanks to Lemma \ref{lm:specC}, we know that $\|C_\abs(W,W) - C_\abs^{\mathrm{lin}}\|_{op} = o(1)$ w.p $1-d^{-1+o(1)}$, where $C_\abs^{\mathrm{lin}} = \beta_1 1_k1_k^\top + \beta_2 WW^\top + \beta_3 I_k = (2/\pi)I_k + \mathcal O(1/d)$. The result then follows immediately.
\end{proof}

% \begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
% \begin{restatable}{cor}{}
% % Suppose the rows $w_1,\ldots,w_k$ are drawn iid uniformly from $\sphere$ of the hidden weights matrix $W \in \mathbb R^{k \times d}$, and 
% % the activation function $\sigma$ is the ReLU.
% For the quadratic activation function $t \mapsto t^2/2$, for sufficiently large $d$ the following hold w.p $1-d^{-1+o(1)}$ over the choice of the hidden weights matrix $W \sim \tau_d^{\otimes k}$
% \begin{itemize}
% \item[(A)] Linearization of nonlinear kernel random $C_\sigma(W)$.
% \begin{eqnarray}
% \|C_\sigma(W) - WW^\top\|_{op} = \mathcal O(d^{-1/2}\log^{0.51} d):
% \end{eqnarray}
% \item[(B)] Estimation of eigenvalues of $C_\sigma(W)$: If $\lambda_{\max} = \lambda_1 \ge \ldots \ge \lambda_k = \lambda_{\min}$ are the eigenvalues of $C_\sigma(W)$ and $\overline{\lambda}_1 \ge \ldots \ge \overline{\lambda}_k $ are the eigenvalues of $WW^\top$, then
% \begin{eqnarray}
% \lambda_j = \overline{\lambda}_j + \mathcal O(d^{-1/2}\log^{0.51} d),\text{ for all }j \in [k].
% \end{eqnarray}

% \item[(C)] Estimation of extreme eigenvalues of $C_\sigma(W)$. We have $\lambda_{\max} = \mathcal O(1)$. Moreover, if $k/d \le \gamma_2 < 1$, then
% \begin{eqnarray}
% \lambda_{\min} = \Omega(1).
% \end{eqnarray}
% \end{itemize}
% \label{cor:Cspecquad}
% \end{restatable}
% \end{mdframed}
% \begin{proof}
% One has $\widetilde{\kappa}_\sigma(t) = t+t^2/(d(d+2))$ for all $t \in [-1,1]$, and so one computes $\beta_1(\widetilde{\kappa}_\sigma)=0$, $\beta_2(\widehat{\kappa})=1$, $\beta_3(\widetilde{\kappa}_\sigma)=0$. Parts (A) and (B) of the proof then follow directly from Lemma \ref{lm:specC}. Part (C) is standard RMT applied to the matrix $WW^\top$.
% \end{proof}


\paragraph{Extending to other homogeneous activation functions.} Inspecting the above proofs of Corollary \ref{cor:Cspecrelu}, we see that to control the extreme singular-values of the kernel random matrix $C_\sigma(W)$, it is sufficient that $\sigma$ verifies the following assumption.
\mytodo{previous statement is outdated and has been moved to much above}
Examples of activation functions for which Condition \ref{cond:relulike} holds include: ReLU, absolute-value, error-function (erf), etc.

We have the following extension of Corollary generalizes both Corollary \ref{cor:Cspecrelu}.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Extreme singular-values of induced kernel $C_\sigma(W)$]{cor}{}
Suppose Condition \ref{cond:relulike} is in order. We have the following
\begin{itemize}
    \item[(A)] Lower-bound on smallest eigenvalue of $C_\sigma(W)$: For sufficiently large $d \asymp k$, if either
\begin{itemize}
\item[(i)] $\beta_3(\widetilde{\kappa}_\sigma) = \Omega(1)$, or
\item[(ii)] $k/d \le \gamma_2 < 1$ and $\beta_2(\widetilde{\kappa}_\sigma)=\Omega(1)$,
\end{itemize}
then it holds w.p $1-d^{-1+o(1)}$ that $\lambda_{\min}(C_\sigma(W) = \Omega(1)$.
\item[(B)] Upper bound on largest eigenvalue of $C_\sigma(W)$: If $d,k \to \infty$ with $k/d \in (0,\infty)$, then $\lambda_{\max}(C_\sigma(W)) = \mathcal O_{\mathbb P}(1)$.

% We now show that $\lambda_{\max}(K(X,X)) = \mathcal O_{\mathbb P}(1)$.
\end{itemize}
\end{restatable}
\label{cor:Cspecrelulike}
\end{mdframed}
\begin{proof}
Direct adaptation of the proof of Corollary \ref{cor:Cspecrelu}.
\end{proof}
% \lorem
% The following result establishes that for large $d$, the robustness $\mathfrak{S}(f_{W,v})$ of random model $f_{W,v} \in \mathcal F_{d,k}(\sigma)$ with $W \sim \tau_d^{\otimes }$, varies as $\|v\|$. This result will be the corner stone for our analysis of random features model.
% \begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
% \begin{restatable}[Control of Sobolev-seminorm of RF model via norm of output weights vector]{thm}{}
% Suppose Condition \ref{cond:relulike} is in order. Then for $k \asymp d$ sufficiently large, it holds w.p $1-d^{-1+o(1)}$ over the choice of the hidden weights matrix $W$, the following hold
% \begin{itemize}
% \item[(A)] Lower-bound: For sufficiently large $d \asymp k$ and if either
% \begin{itemize}
% \item[(i)] $\beta_3(\widetilde{\kappa}_\sigma) = \Omega(1)$, or
% \item[(ii)] $k/d \le \gamma_2 < 1$ and $\beta_2(\widetilde{\kappa}_\sigma)=\Omega(1)$,
% \end{itemize}
% then it holds w.p $1-d^{-1+o(1)}$ over $W$ that $\mathfrak{S}(f_{W,v}) = \Omega(\|v\|)$.
% \item[(B)] Upper-bound: In the limit $d,k \to \infty$ such that $k/d \in (0,\infty)$, it holds that
% $$
% \mathfrak{S}(f_{W,v}) = \mathcal O_{\mathbb P}(\|v\|).
% $$
% \end{itemize}
% \label{thm:relusob}
% \end{restatable}
% \end{mdframed}
% \begin{proof}
% We know from Corollary \ref{cor:Cspecrelulike} that under Condition \ref{cond:relulike}, it holds w.p $1-d^{-1+o(1)}$ that
% \begin{itemize}
% \item[--] $\lambda_{\max}(C_\sigma(W)) = \mathcal O(1)$, and
% \item[--] if $\beta_3(\widetilde{\kappa}_\sigma)>0$ or $k/d \le \gamma_2 < 1$ and $\beta_2(\widetilde{\kappa}_\sigma)$, then
% $\lambda_{\min}(C_\sigma(W)) = \Omega(1)$.
% \end{itemize}
Follows directly from Theorem \ref{thm:analytic} (more specifically, refer to \eqref{eq:sandwitch}) and Corollary \ref{cor:Cspecrelulike}.
% On the other hand, standard random matrix theory (cite Vershynin and Rudelson 20XY) guarantees that $\lambda_{\max}(WW^\top) = \mathcal O(1)$ w.p $1-e^{-\Omega(d)}$, and so we deduce from \eqref{eq:approxeig} that $\lambda_{\max}(C_\sigma(W)) = \mathcal O(1)$ w.p $1-d^{-1+o(1)}$, and the result follows from Theorem \ref{thm:analytic} and the righmost side of \eqref{eq:sandwitch}.
% \end{proof}

\subsection{Law of robustness for finite-width random features models}
\lorem


==> preliminaries.tex <==
\section{Warmup: Analysis of ordinary linear models}
\label{sec:ordinary}
% \lorem 
 Let us forget about neural networks for a moment. 
 
 \subsection{Chaos in linear regression}
% \lorem

Let $n,d \to \infty$ with $n/d \to \gamma \in (0,\infty)$. Let $X$ be a random $n \times d$ matrix with entries from $N(0,1/d)$ and let $y$ be a random vector in $\mathbb R^n$ independent of $X$, with iid entries uniformly distributed on $\{\pm 1\}$. To simplify arguments, we may WLOG temporality assume that $y_1,\ldots,y_n \sim N(0,1)$.

Now, for a ridge penalty $\lambda > 0$ let $Q_\lambda(\omega) := (\omega + n\lambda I_n)^{-1}$ and set $\widehat{\beta}_\lambda := Q_\lambda(XX^\top)X^\top y \in \mathbb R^d$, the unique solution to the (random) ridge-regression problem
\begin{eqnarray}
\begin{split}
\arg\min_{\beta \in \mathbb R^d}\frac{1}{2n}\|y-X\beta\|^2 + \lambda \|\beta\|^2.
\end{split}
\label{eq:ridge}
\end{eqnarray}
It is clear by definition that, conditioned on the design matrix $X$ the regressor $\widehat{\beta}_\lambda$ has centered multivariate distribution with covariance matrix $R_\lambda(X^\top X)=Q_\lambda(X^\top X)X^\top XQ_\lambda(X^\top X)$, where
$Q_\lambda(S) := (S+n\lambda)^{-1}$,
and so one has
\begin{eqnarray}
\|\widehat{\beta}_\lambda\|^2 \to  \trace(R_\lambda(X^\top X))\text{ almost-surely.}
\label{eq:betanorm}
\end{eqnarray}
% where $\mbox{tr}_d(R_\lambda(XX^\top))$ is the trace of $R_\lambda(XX^\top)$ divided by $d$.
% Since $XX^\top$ is a "free random variable" (in the sense of free probability), and $R_\lambda(XX^\top)$ is a rational expression in $\omega=XX^\top$, one would expect $\|\widehat{\beta}_\lambda\|^2$ to have a complete analytic description via free probability.

{\bfseries Question:}\emph{ How large can the $L_2$-norm of the regressor $\widehat{\beta}_\lambda$ be ?}

The following theorem provides the exact asymptotic expansion of $\|\widehat{\beta}_\lambda\|$.

\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Asymptotics of norm of ridge(less) regressors]{thm}{ridgelimits} Consider the ridge-regression problem \eqref{eq:ridge} in the regime where $n,d \to \infty$ with $n/d \to \gamma \in (0,\infty)$. Let $\lambda \ge 0$ be the ridge penalty parameter, possible depending on $n$ (or equivalently, on $d$). Then, it holds that
\begin{eqnarray}
\begin{split}
\frac{\|\widehat{\beta}_\lambda\|^2}{n} &= \frac{\gamma-n\lambda + 1}{2\gamma\sqrt{(\gamma-n\lambda + 1)^2 + 4n\lambda}}-\frac{1}{2\gamma}+o_{\mathbb P}(1).
\end{split}
\label{eq:generalform}
\end{eqnarray}
% Furthermore, the memorization error of the regressor is given by
% \begin{eqnarray}
% \frac{\|y-X\widehat{\beta}_\lambda\|^2}{n}=
% \end{eqnarray}
In particular, we have the following extreme cases.
\begin{itemize}
    \item[(A)] (Norm of small ridge regressor) If $\lambda=o(1/n)$, then
    \begin{eqnarray}
    \begin{split}
    \dfrac{\|\widehat{\beta}_\lambda\|^2}{n \land d} = \frac{1}{|1-\gamma|}+o_{\mathbb P}(1).
    \end{split}
    \end{eqnarray}
    Moreover, the memorization error of $\widehat{\beta}_\lambda$ satisfies
    \begin{eqnarray}
    \frac{\|y-X\widehat{\beta}_\lambda\|^2}{n} = (1-\frac{1}{\gamma})_+ + o_{\mathbb P}(1).
    \end{eqnarray}
    \item[(B)] (Norm of large ridge regressor) If $\lambda=\omega(1/n)$, then
    \begin{eqnarray}
    \frac{\|\widehat{\beta}_\lambda\|^2}{n} = o_{\mathbb P}(1).
    \label{eq:infiniteridge}
    \end{eqnarray}
    Moreover, the memorization error of $\widehat{\beta}_\lambda$ satisfies
    \begin{eqnarray}
    \frac{\|y-X\widehat{\beta}_\lambda\|^2}{n} = 1 + o_{\mathbb P}(1).
    \end{eqnarray}
\end{itemize}
\label{thm:ridgelimits}
\end{restatable}
\end{mdframed}
\paragraph{Consequences of Theorem \ref{thm:ridgelimits}.} We draw the following important consequences:
\begin{itemize}
    \item[--] \emph{Nonrobustness "small" regressor $\lambda = o(1/n)$.}
    Such a regressor memorizes generic data $\mathcal D_n$ and its $L_2$-norm is given by $\|\widehat{\beta}_{\lambda}\| = \Theta_{\mathbb P}(\sqrt{n})$; a small perturbation (i.e of order $\Theta (1)$) in the input of the linear model $x \mapsto x^\top \widehat{\beta}_{\lambda}$ will lead to a change of order $\sqrt{n}$ in the output prediction, implying an unbearable level of nonrobustness.
    
    \item[--] \emph{Catastrophic nonrobustness close to interpolation threshold.} Worst still, close to the interpolation threshold $d=n$ (i.e $\gamma \to 1$), we obtain $\|\widehat{\beta}_\lambda\| = \omega_{\mathbb P}(\sqrt{n})$.
    
    \item[--] \emph{Robustness of "large" ridge regressor $\lambda = \omega(1/n)$.} On the other hand, even a small ridge penalty of order $\lambda=\Omega(1/\sqrt{n})$ is sufficient to ensure $\|\widehat{\beta}_\lambda\| = o_{\mathbb P}(\sqrt{n})$ almost-surely.
\end{itemize}
We shall see later in the manuscript that these observations remain true even in nonlinear random features and neural tangent kernel regimes.

\subsection{Nonasymptotic analysis of robustness of ridgeless regression}
For a fixed vector $w \in \mathbb R^d$ of parameters, we consider a linear model $f_w:\mathbb R^d \to \mathbb R$ defined by $f_w(x):=x^\top w$. Note that $f_w$ is equivalent to a single hidden neuron (i.e $k=1$) with no activation function, i.e $f_w \in \mathcal F_{d,1}(\sigma_{\mbox{id}})$. % The expectation of $f_{w}(x)$ on the unit-sphere is $\mathbb E_{x \sim \tau_d}[f_w(x)] = 0$. Furthermore, one computes
For $x \sim \tau_d$, one computes
\begin{eqnarray}
\mathbb E_x \|\nabla_{\sphere} f_w(x)\|^2 = \|w\|^2-\mathbb E_x (x^\top  w)^2 = \|w\|^2 - \trace(ww^\top \cov(x)) = (1-1/d)\|w\|^2.
\label{eq:linpoincare}
\end{eqnarray}
% \begin{eqnarray}
% \begin{split}
% \var_{\tau_d}(f_w) &= \|f_w-\mathbb E_{x \sim \tau_d}[f_w(x)]\|_{L^2(\tau_d)}^2
% = \|f_w\|_{L^2(\tau_d)}^2 = \mathbb E_{x \sim \tau_d}[(x^\top w)^2]\\
% &= \|w\|^2\cdot \mathbb E_{x \sim \tau_d}[x^\top x] = \frac{\|w\|^2}{d}.
% \end{split}
% \label{eq:linearsphere}
% \end{eqnarray}
% Thus, by the Poincar\'e inequality \eqref{eq:poincare}, we deduce that
% \begin{eqnarray}
% \label{eq:linpoincare}
% \Lip_{\sphere}(f_w) \ge \|\nabla_{\sphere} f_w\|_{L^2(\tau_d)} \gtrsim \|w\|.
% \end{eqnarray}
It remains to lower bound $\|w\|$. Now, suppose the model $f_w$ memorizes the generic dataset $\mathcal D_n$ (in the sense of Definition \ref{df:memo}). Then $n\epsilon \ge \|\widehat{y}-y\|^2 \ge \|y\|^2 - 2y^\top\widehat{y} = n - 2 y^\top\widehat{y}$, where $y:=(y_1,\ldots,y_n)$ if the array of labels in the $\mathcal D_n$, and $\widehat{y}:=(f_w(x_1),\ldots,f_w(x_n))$ is the array of predictions of $f_w$ on $\mathcal D_n$. Thus, we derive the following inequalities
\begin{eqnarray}
\label{eq:neuron}
\frac{n}{2\|w\|} \le \frac{y^\top\widehat{y}}{\|w\|} = \sum_{i=1}^n y_i \frac{x_i^\top w}{\|w\|} \le \|X^\top y\|. % \le \sup_{u \in \sphere}\sum_{i=1}^n y_i \sigma(x_i^\top u).
\end{eqnarray}
In order to bound the RHS of the above inequalities, we will need the following lemma (proved in the appendix), which roughly states that a single neuron cannot be too correlated with generic data. Also see ~\cite{bubecknetsize} for an expectation version of this result.
\begin{restatable}[Maximal correlation of a neuron]{lm}{turbo}
Suppose $n = \Omega((\log d)^C)$ for some $C>0$. If $\sigma:\mathbb R \to \mathbb R$ is $1$-Lipschitz, then for large $d$ it holds w.p $1-d^{-\Omega(1)}$ over $\mathcal D_n$ that
\begin{eqnarray}
\underset{w \in \mathbb R^d}{\sup}\;\sum_{i=1}^n \dfrac{y_i\sigma(x_i^\top w)}{\|w\|}=\mathcal O(\sqrt{n}).
 \end{eqnarray}
 % \begin{itemize}
% \item[(A)] If $d \le \sqrt{n}$, then it holds w.p $1-e^{-\Omega(\sqrt{n})}$ over $\mathcal D_n$ that $Z = \mathcal O(\sqrt{n})$.
% \item[(B)] If $d > \sqrt{n}$, then it holds w.p $1-e^{-\Omega(d)}$ over $\mathcal D_n$ that $Z = \mathcal O(n/d)$.
 % \end{itemize}
\label{lm:turbo}
\end{restatable}
By Lemma \ref{lm:turbo}, w.p $1-d^{-\Omega(1)}$ the rightmost side of \eqref{eq:neuron} is $\mathcal O(\sqrt{n})$, and so $\|w\| = \Omega(\sqrt{n})$ w.p $1-d^{-\Omega(1)}$.
Combining with \eqref{eq:linpoincare}, we deduce the following result.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}{thm}{}
If $n=\Omega((\log d)^C)$ for some $C>0$, it holds w.p $1-d^{-\Omega(1)}$  over $\mathcal D_n$ that any linear model $f_w \in \mathcal F_{d,1}(\sigma_{\text{id}})$ which memorizes $\mathcal D_n$ satisfies $\mathfrak{S}(f_w) = \Omega(\sqrt{n})$.
\label{thm:linthm}
\end{restatable}
\end{mdframed}
Note that the above theorem is not void, since the least-squares model is at least one such model (as it indeed memorizes the generic dataset with probabilit $1-o(1)$).

\paragraph{Tightness of the lower-bound.} Suppose $n = \mathcal O(d)$. There might be different possible choices for the parameter $w \in \mathbb R^d$ of the candidate linear model $f_w$ which perfectly memorizes the generic dataset $\mathcal D_n$, but the one with minimal variance is $w := X^\dagger y = X^\top(XX^\top)^{-1}y$, where $X \in \mathbb R^{n \times d}$ is the design matrix, the $i$th row of which is $x_i$. It was shown in \cite{lor} using standard random matrix theory (to upper bound the spectral norm of $X$), that
$\Lip_{\sphere}(f_w) =\mathcal O(\sqrt{n})$ w.p $1-e^{-\Omega(d)}$.

% \section{Proof of Conjecture \ref{conj:bubeck}}
% \begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
% \begin{restatable}{thm}{}
% Let the activation function be $\psi$ one Lipschitz. It holds w.p $1-e^{-\Omega(\sqrt{n} \lor d})$ that any $f \in \mathcal F_{d,k}(\sigma)$ which memorizes generic data $\mathcal D_n$ must satisfy
% \begin{eqnarray}
% \Lip_{\sphere}(f) = \Omega(\frac{\sqrt{n} \land d}{\sqrt{k}}).
% \end{eqnarray}
% \end{restatable}
% \end{mdframed}
% \begin{proof}
% By, definition, we have
% $$
% \Lip_{\sphere}(f)^2 \ge \max_{i \in [n]}\|\nabla_{\sphere} f(x_i)\|^2
% $$
% \end{proof}


==> pure_nonlinear.tex <==
\subsection{Law of robustness for purely nonlinear RF models in proportional scaling regime}
\begin{restatable}[Gaussian equivalent linear model -- Corollary 6 of \cite{Hastie2019}]{prop}{}
\label{prop:hastie}
Under Condition \ref{cond:purelynonlin}, in the limit $n,d,k \to \infty$ according to the proportionate regime \eqref{eq:proportionate}, if $\mu_0^2 = \mu_1^2 = 0$, then the empirical distribution of the eigenvalues of the nonlinear gram matrix $Z^\top Z=\sigma(XW^\top)\sigma(XW^\top)^\top \in \mathbb R^{k \times k}$ converges weakly and in $L^1$, to the Marchenko-Pastur distrbution with parameter $\gamma$.
\end{restatable}
An example of such an activation function is the shifted asoblute-value $\sigma(t) : =a(|t|-b)$. The following result is one of our main contributions, and identifies a new regime in Conjecture \ref{conj:bubeck}. The result also explicitly outlines quantitative tradeoffs between memorization and robustness.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Nonrobust memorization in the random features regime]{thm}{}
Consider the random features model $\widehat{f}_{\rf}$ and suppose Conditions \ref{cond:relulike} and \ref{cond:purelynonlin} are in action. In the limit when $n,d,k \to \infty$ according to proportional scaling \eqref{eq:proportionate}, it holds that
\begin{itemize}
\item {\bfseries Memorization.} The ridgeless random features model $\widehat{f}_{\rf}$ memorizes $\mathcal D_n$ almost-surely. More precisely, for a ridge parameter $\lambda \ge 0$, the MSE error of the ridged random features model $\widehat{f}_{\rf,\,\lambda}$ is asymptotically given by
\begin{eqnarray}
\mathrm{MSE}(\widehat{f}_{\rf,\; \lambda}) = \begin{cases}(1-\gamma)_+ + o_{\mathbb P}(1),&\mbox{ if }\lambda=o(1/n),\\
1 + o_{\mathbb P}(1),&\mbox{ if }\lambda = \omega(1/n).
\end{cases}
\end{eqnarray}
\item {\bfseries Nonrobustness.} Recall that $\gamma := \lim n/k \in (0,\infty)$ in the proportional scaling \eqref{eq:proportionate}. We have the asymptotic estimates
\begin{eqnarray}
% \Lip_{\sphere}(\widehat{f}_\rf) \ge 
\mathfrak{S}(\widehat{f}_{\rf}) =
\begin{cases}
\Theta_{\mathbb P}(\sqrt{n}),&\mbox{ if }\lambda = o(1/n),\;\gamma \ne 1,\\
\omega_{\mathbb P}(\sqrt{n}),&\mbox{ if }\lambda=o(1/n),\,\gamma = 1,\\
o_{\mathbb P}(\sqrt{n}),&\mbox{ if }\lambda=\omega(1/n).
\end{cases}
\end{eqnarray}
\end{itemize}
\label{thm:nonrobRF}
\end{restatable}
\end{mdframed}
Notice the peak in the nonrobustness at $\gamma=1$ (i.e $k/n \to 1$) which occurs for small regularization $\lambda \ll 1/n$ and disappears for $\lambda \gg 1/n$.
We see that the only hope for trading between robustness and goodness of fit is perhaps to regularize the estimation of the output weights vector with ridge parameter $\lambda \asymp 1/n$. A fine-grained analysis of this is left for future work.

We will need the following lemma from ~\cite{Dobriban2018} (see Lemma 7.6 therein).
\begin{restatable}[Concentration of double-random quadratic forms ~\cite{Dobriban2018}]{lm}{}
Let $Y_n:=(y_1,\ldots,y_n)$ be an iid sequence of random variables such that
 $$
 \mathbb E [y_1] = 0,\;\mathbb E|y_1|^2 = 1,\;\mathbb E|y_1|^{4+\epsilon} < \infty,
 $$
 for some absolute constant $\epsilon>0$.
 Let $A_n$ be an $n \times n$ random (or deterministic) matrix independent of the $y_i$'s, such that $\sup_n \|A_n\|_{op} \le C <  \infty$ w.p $1$. Then, it holds that $n^{-1}Y_n^\top A_n Y_n - n^{-1}\trace(A_n) \to 0$ a.s. In particular, it holds that
\begin{eqnarray}
 n^{-1}Y_n^\top A_n Y_n = n^{-1}\trace(A_n) + o_{\mathbb P}(1).
\end{eqnarray}
\end{restatable}
\begin{proof}[Proof of Theorem \ref{thm:nonrobRF}]
% Thanks to the Proposition \eqref{prop:hastie}, we are basically in the setting of Theorem \ref{thm:linthm}.
The proof is divided in to several steps.

\emph{-- Memorization error of $\widehat{f}_\rf$.} % WLOG, suppose $\gamma > 1$; otherwise replace $\gamma$ by $1/\gamma$, and $Z$ by $Z^\top$ in the computations below \mytodo{Too hand-wavy!}.
Thanks to Proposition \ref{prop:hastie}, the eigenvalue statistics of the model with design matrix $\sigma(XW^\top)$ are equivalent to the eigenvalue statistics of model with gaussian features and design matrix with $n/d \to \gamma_1$.
Let $\lambda_1 \ge \lambda_2 \ge \ldots \ge \lambda_{\rank (Z)}$ be the eigenvalues of $Z^\top Z$. One computes
\begin{eqnarray}
\begin{split}
\mathrm{MSE}(\widehat{f}_{\rf,\lambda}) &= \dfrac{1}{n}\|y-Z\widehat{v}_{\rf,\lambda}\|^2 = \frac{1}{n}y^\top(I-Z(Z^\top Z + \lambda n)^{-1} Z^\top)^2 y\\
&= \dfrac{1}{n}\trace((I-Z(Z^\top Z + n\lambda)^{-1}Z^\top)^2) + o_{\mathbb P}(1)\\
&=1-\frac{2}{n}\trace(Z^\top Z(Z^\top Z + n\lambda)^{-1}) + \frac{1}{n}\trace((Z^\top Z(Z^\top Z + n\lambda)^{-1})^2)+o_{\mathbb P}(1)\\
&= 1 - \frac{2}{n}\sum_{j=1}^k \frac{\lambda_i}{\lambda_i + n\lambda} + \frac{1}{n}\sum_{j=1}^k \frac{\lambda_i^2}{(\lambda_i+n\lambda)^2}+o_{\mathbb P}(1)\\
&=1-2\int \frac{t}{t + n\lambda}\diff\mu^{\MP}_\gamma(t) + \int \frac{t^2}{(t+n\lambda)^2}\diff\mu^\MP_\gamma(t)+o_{\mathbb P}(1)\\
&=
\begin{cases}
(1-1/\gamma)_+ + o_{\mathbb P}(1),&\mbox{ if }\lambda = o(1/n),\\
1+o_{\mathbb P}(1),&\mbox{ if }\lambda = \omega(1/n).
\end{cases}
\end{split}
\end{eqnarray}
where in the second step (the a.s convergence), we have used the fact the the spectrum of the random matrix $(I-Z(Z^\top Z + \lambda n \lambda)^{-1}Z^\top)^2$ is uniformly bounded\footnote{That is $c \le \lambda_{k} \le \lambda_1 \le C$ for absolute constants $c,C \in (0,\infty)$.} a.s (since thanks to Proposition \ref{prop:hastie}, $\lambda_{\max}(Z^\top Z) \le (1+\sqrt{\gamma})^2 + o_{\mathbb P}(1)$), to invoke ~\cite[Lemma 7.6]{Dobriban2018}. % , and the other steps parallel the steps in the proof of Theorem \ref{thm:linthm}.

\emph{-- The asymptotics of $\|\widehat{v}_{\rf,\lambda}\|$.} % We will use Theorem \ref{thm:relusob}. For this, we need to estimate $\|\widehat{v}_\lambda\|^2$.
Similarly to the previous computation, we have
\begin{eqnarray}
\begin{split}
\frac{1}{n}\|\widehat{v}_{\rf,\lambda}\|^2&=\frac{1}{n}y^\top Z(Z^\top Z + n\lambda)^{-2}Z^\top y=\frac{1}{n}\trace(Z^\top Z(Z^\top Z + n\lambda)^{-2}) + o_{\mathbb P}(1)\\
&= \frac{1}{n}\sum_{j=1}^k \frac{\lambda_i}{(\lambda_i + n\lambda)^2}+o_{\mathbb P}(1) = \int \frac{t}{(t+n\lambda)^2}\diff\mu^\MP_\gamma(t) + o_{\mathbb P}(1)\\
&= \frac{\gamma-n\lambda + 1}{2\gamma\sqrt{(\gamma-n\lambda + 1)^2 + 4n\lambda}}-\frac{1}{2\gamma}+o_{\mathbb P}(1)\\
&=
\begin{cases}
\dfrac{\gamma \land 1}{|1-\gamma|} + o_{\mathbb P}(1),&\mbox{ if }\lambda=o_{\mathbb P}(1/n),\\
o_{\mathbb P}(1),&\mbox{ if }\lambda=\omega(1/n).
\end{cases}
\end{split}
\end{eqnarray}
% The first part is proved by Lemma \ref{lm:gammafit}. We now prove that $\|\widehat{v}\| = \Theta(\sqrt{n})$ in probability and conclude by invoking Theorem \ref{thm:relusob}.
% Let $\mathcal E_n$ be the event that the linearization \eqref{eq:linearize} holds. Note that $\mathbb P(\mathcal E_n)=1-o(1) \to 1$ and conditioned on $\mathcal E_n$, we have by virtue of $\gamma < 1$,
% $$
% c \le \lambda_{\min}(Z^\top Z) \le \lambda_{\max}(Z^\top Z) \le C,
% $$
% for some universal / absolute constants $c,C \in (0,\infty)$. Conditioned on $\mathcal E_n$, $Z$ has independent rows and the unique solution for the output weights vector $\widehat{v}$ for the random features regressor is given by $\widehat{f}_{\rf}$ $\widehat{v}=Z^\dagger y = (Z^\top Z)^{-1}Z^\top y \in \mathbb R^{k}$. Thus, conditioned on the event $\mathcal E_n$, the expected value of $n^{-1}\|\widehat{v}\|^2$ is given by
% \begin{eqnarray*}
% \begin{split}
% \mathbb E[n^{-1}\|\widehat{v}\|^2 \mid \mathcal E_n] &= \frac{1}{n}\mathbb E[\|(Z^\top Z)^{-1}Z^\top y\|^2 \mid \mathcal E_n] = \frac{1}{n}\mathbb E[y^\top Z(Z^\top Z)^{-2} Z^\top y \mid \mathcal E_n]\\
% &=\frac{1}{n}\trace(Z (Z^\top Z)^{-2} Z^\top \cov(y)) = \frac{1}{n}\trace((Z^\top Z)^{-1}) \in [C^{-1},c^{-1}],
% \end{split}
% \end{eqnarray*}
% Similarly, for the conditional variance, one computes
% \begin{eqnarray*}
% \begin{split}
% \var(n^{-1}\|\widehat{v}\|^2 \mid \mathcal E_n) &= \frac{1}{n^2}\var(y^\top Z(Z^\top Z)^{-2}Z^\top y \mid \mathcal E_n)=\frac{2}{n^2}\trace(Z(Z^\top Z)^{-2} Z^\top Z(Z^\top Z)^{-2}Z)\\
% &=\frac{2}{n^2}\trace((Z^\top Z)^{-2}) \le \frac{2c^{-2}}{n} = \mathcal O(\frac{1}{n}).
% \end{split}
% \end{eqnarray*}
% Thus for every $t > 0$, one computes
% \begin{eqnarray}
% \begin{split}
% \mathbb P(-t + C^{-1} \le n^{-1}\|\widehat{v}\|^2 \le c^{-1} + t) &\ge \mathbb P(|n^{-1}\|\widehat{v}\|^2-\mathbb E[ n^{-1}\|\widehat{v}\|^2 \mid \mathcal E_n] \le t)\\
% &\ge \mathbb P(\mathcal E_n)\mathbb P(|n^{-1}\|\widehat{v}\|^2-\mathbb E[ n^{-1}\|\widehat{v}\|^2 \mid \mathcal E_n] \le t \mid \mathcal E_n)\\
% &\ge \mathbb P(\mathcal E_n)(1-\frac{\var(n^{-1}\|\widehat{v}\|^2 \mid \mathcal E_n)}{t^2})\\
% &=\mathbb P(\mathcal E_n)(1-\mathcal O(\frac{1}{t^2n}))\\
% &=(1-o(1))(1-\mathcal O(\frac{1}{t^2n})) \to 1,
% \end{split}
% \end{eqnarray}
% from which we conclude that $\|\widehat{v}\| = \Theta_{\mathbb P}(\sqrt{n})$.
Combining this with inequality \eqref{eq:relusob} of Theorem \ref{thm:relusob} then completes the proof.
\end{proof}


==> rf_linear_interp.tex <==
\subsection{Nonrobust memorization in RF models in linear interpolation regime} 
We now depart from the assumption that $n$, $d$, and $k$ go to infinity at the same rate (the so-called quadratic interpolation regime). We place ourselves in the so-called linear interpolation regime, where $kd$ is only larger than $n$ (modulo log factors).
% Note that Theorem \ref{thm:nonrobRF} is $\sqrt{k}$ stronger than the $\Omega(\sqrt{n/k})$ bound predicted by Conjecture \ref{conj:bubeck}. We managed to get such an improvement by considering the infinite dataset limit $n \to \infty$ to argue that $\|\widehat{v}\| = \Omega(\sqrt{n})$, which then ensures $\mathfrak{S}(f)$ thanks to Theorem \ref{thm:relusob}. In case the size $n$ of the dataset is fixed, i.e $n \not \to \infty$, the arguments in XXX may fail. In this case, we only manage to ensure that $\|\widehat{v}\| = \Omega((\sqrt{n}\land d)/\sqrt{k})$ w.p $1-o(1)$, thanks to the following lemma.

For simplicity of the following results, assume $n = \Omega((\log d)^C)$.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}{lm}{khintchine}
Let $\sigma$ be a $1$-Lipschitz activation function. If $n = \Omega((\log d)^C)$ for some constant $C > 0$, then w.p $1-d^{-\Omega(1)}$ over the choice of $\mathcal D_n$, any $f = f_{W,v}\in \mathcal F_{d,k}(\sigma)$, which memorizes the generic dataset $\mathcal D_n$ must satisfy
\begin{eqnarray}
\|v\| \ge \Omega\left(\frac{1}{M}\sqrt{\frac{n}{k}}\right),
\label{eq:vnorm}
\end{eqnarray}
where $M := \sup_{j \in [k]}\|w_j\|$.
\label{lm:khintchine}
\end{restatable}
\end{mdframed}
Note that possible dependence on the input dimension $d$ is implicitly hidden $\|W\|_{op}$, the spectral norm of the hidden weights matrix $W \in \mathbb R^{k \times d}$. A weaker version\footnote{The authors proved \eqref{eq:vnorm} only with positive probability.} thereof was proved in \cite[Theorem 3]{lor}.

\begin{proof}[Proof of Lemma \ref{lm:khintchine}]
The proof parallels that of \cite[Theorem 3]{lor} and \cite[Proposition 1]{bubeck2018}, which reduce the problem to that of bounding the supremum of a certain empirical process. Indeed, by basic manipulations and the Cauchy-Schwarz inequality, we have
\begin{eqnarray}
\sqrt{k}\|v\| M = \sqrt{k}\|v\| \max_{1 \le j \le k}\|w_j\| \ge \|v\|_1 \max_{1 \le j \le k}\|w_j\| \ge \sum_{j=1}^k |v_j|\|w_j\|=:\eta(f),
\end{eqnarray}
% where $\eta(f)$ is the complexity measure defined in \eqref{eq:bartlettnorm}.
We deduce that
\begin{eqnarray}
\label{eq:eta}
\|v\| \ge \dfrac{\eta(f)}{M\sqrt{k}}.
\end{eqnarray}
Thus, it suffices to prove that $\eta(f) =\Omega(\sqrt{n} \land d)$ with the desired probability. To this end, define $\widehat{y} \in \mathbb R^n$ by setting $\widehat{y}_i := f(x_i) = \sum_{j=1}^k v_j\sigma(x_i^\top w_j)$ for all $i \in [n]$. Since the generic dataset $\mathcal D_n$ is memorized by $f$ (refer to Definition \ref{df:memo}), it holds that
$n/2 \ge \|\widehat{y}-y\|^2 \ge \|y\|^2 - 2 \widehat{y}^\top y=n-2\widehat{y}^\top y$, and so one computes
\begin{eqnarray*}
\begin{split}
\frac{n}{4} &\le \widehat{y}^\top y = \sum_{j=1}^k\sum_{i=1}^n y_i v_j \sigma(x_i^\top w_j) \le \sum_{j=1}^k \sum_{i=1}^ny_i\frac{\sigma(x_i^\top w_j)}{\|w_j\|} v_j\|w_j\|\\
& \overset{\text{CS}}{\le} \eta(f)\cdot \max_{1 \le j \le k}\sum_{i=1}^n y_i\frac{\sigma(x_i^\top w_j)}{\|w_j\|}
% = \eta(f)\cdot \max_{1 \le j \le k}\sum_{i=1}^n y_i\sigma(x_i^\top w_j/\|w_j\|) \\
\le \eta(f)\cdot \underbrace{\sup_{w \in \mathbb R^d}\sum_{i=1}^n y_i \frac{\sigma(x_i^\top w)}{\|w\|}}_{A},
 % &\overset{(ii)}{=} \eta(f)\cdot \sup_{w \in \sphere}\sum_{i=1}^n y_i\sigma(x_i^\top w),
\end{split}
\end{eqnarray*}
 i.e $\eta(f) \ge \dfrac{n}{4A}$.
% where (i) is due to Cauch-Schwarz inequality and (ii) is because the activation function $\sigma$ was assumed to be positive $1$-homogeneous. 
By Lemma \ref{lm:turbo}, we know that $A = \mathcal O(\sqrt{n} \lor n/d)$ w.p $1-e^{-\Omega(\sqrt{n} \lor d)}$.
% Now, taking expectations w.r.t $y_1,\ldots,y_n$  and combining with standard Rademacher arguments gives
% \begin{eqnarray*}
% \begin{split}
% \frac{n}{2\eta(f)} &\le \mathbb E_y\sup_{w \in \mathbb R^d}\sum_{i=1}^n y_i \frac{\sigma(x_i^\top w)}{\|w\|} \le \|\sigma\|_{\Lip}\cdot \mathbb E_y\sup_{w \in \mathbb R^d}\sum_{i=1}^n y_i \frac{x_i^\top w}{\|w\|}\\
% &\le \|\sigma\|_{\Lip}\cdot\left(\sum_{i=1}^n \|x_i\|^2\right)^{1/2} = \|\sigma\|_{\Lip}\cdot \sqrt{n}.
% \end{split}
% \end{eqnarray*}
% Thus, taking $\tau = \sqrt{n}$ we obtain that w.p $1-e^{-\Omega(\sqrt{n} )}$,
% $$
% R_n = \begin{cases}\mathcal O(\sqrt{n}),&\mbox{ if }d \le n,\\\mathcal O(\frac{n}{\sqrt{d}}),&\mbox{else.}\end{cases}
% $$
Therefore $\eta(f)  \ge \dfrac{n}{4Z} =\Omega(\sqrt{n} \land d)$ w.p $1-e^{-\Omega(\sqrt{n} \lor d )}$.
The desired result then follows immediately upon combining this lower-bound with \eqref{eq:eta}.
\end{proof}

Equipped with Lemma \ref{lm:khintchine}, we can now establish a finite-sample version of Theorem \ref{thm:nonrobRF}. This is one of our main contributions.
\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Nonrobust memorization in finite-width random features regime]{thm}{}
Suppose the activation function $\sigma$ is $1$-Lipschitz with $\sigma(0)=0$. % Suppose $n,d,k \to \infty$ such that $k=\Theta(d)$.
% Then, the following hold.
% \begin{itemize}
% \item {\bfseries Memorization.} If $k=\Omega(n/d)$, then the random features model $\widehat{f}_{\rf}$ memorizes $\mathcal D_n$ w.p $1-e^{-\Omega(d)}$ (i.e w.r.t randomness in $\mathcal D_n$ and $W$).
% \item {\bfseries Nonrobustness.}
For sufficiently large $d$ with $k = \Theta(d)$ and $n = \Omega((\log d)^C)$, it holds w.p $1-d^{-1+o(1)}$ over the choice of $\mathcal D_n$ and $W$ that
\begin{itemize}
    \item {\bfseries Memorization.} $\widehat{f}_{\rf}$ memorizes $\mathcal D_n$.
    \item {\bfseries Nonrobustness.} The following lower-bound holds
\begin{eqnarray}
% \Lip_{\sphere}(\widehat{f}_{\rf}) \ge
\mathfrak{S}(\widehat{f}_\rf) = \Omega(\sqrt{\frac{n}{k}}).
\end{eqnarray}
\end{itemize}
% \end{itemize}
\label{thm:nonrobRFFiniteSample}
\end{restatable}
\end{mdframed}
% Of course the bound in the above theorem only becomes interesting when $n \ll k$ (i.e $k$ is larger than any fixed constant times $d$ or $n$). This is the case for example, in the so-called sub-linear parametrization regime where $n = \widetilde{\Omega}(kd)$.
\begin{restatable}{rmk}{}
\label{rmk:memobubeck}
Under the regime in Theorem \ref{thm:nonrobRFFiniteSample}, it is well-known that $\widehat{f}_{\rf}$ does memorize the generic dataset $\mathcal D_n$ w.p $1-e^{-\Omega(d)}$, provided there are $k = \Omega(n/d)$ hidden neurons. See ~\cite{bubecknetsize}, for example. Our contribution in here is to prove that this memorization is nonrobust.
\end{restatable}
\begin{proof}[Proof of Theorem \ref{thm:nonrobRFFiniteSample}]
Thanks to Theorem \ref{thm:relusob}, we know that if $k=\mathcal O(d)$ the it holds w.p $1-d^{-1+o(1)}$ over the choice of $W$ that
\begin{eqnarray}
% \Lip_{\sphere}(\widehat{f}_{\rf}) \ge 
\mathfrak{S}(\widehat{f}_\rf) = \Theta(\|\widehat{v}\|).
\label{eq:half}
\end{eqnarray}
Now, thanks to Remark \ref{rmk:memobubeck}, $\widehat{f}_{\rf}$ memorizes $\mathcal D_n$ w.p $1-e^{-\Omega(d)}$
On the other hand, invoking Lemma \ref{lm:khintchine} with $M=\|W\|_{op}$ gives $\|\widehat{v}\| = \Omega(\|W\|_{op}^{-1}\sqrt{n/k})$. Also, because $k = \mathcal O(d)$ and $W \sim N(0,1/d)^{k \times d}$, standard RMT tells us that $\|W\|_{op} = \mathcal O(1)$ w.p $1-e^{-\Omega(d)}$, and the result follows immediately upon combining with \eqref{eq:half}.
\end{proof}
